Eridanus III and DELVE 1: Carbon-rich Primordial Star Clusters or the Smallest Dwarf Galaxies?

We present spectroscopy of the ultra-faint Milky Way satellites Eridanus III (Eri III) and DELVE 1. We identify eight member stars in each satellite and place non-constraining upper limits on their velocity and metallicity dispersions. The brightest star in each object is very metal-poor, at [Fe/H] = -3.1 for Eri III and [Fe/H] = -2.8 for DELVE 1. Both of these stars exhibit large overabundances of carbon and very low abundances of the neutron-capture elements Ba and Sr, and we classify them as CEMP-no stars. Because their metallicities are well below those of the Milky Way globular cluster population, and because no CEMP-no stars have been identified in globular clusters, these chemical abundances could suggest that Eri III and DELVE 1 are dwarf galaxies. On the other hand, the two systems have half-light radii of 8 pc and 6 pc, respectively, which is more compact than any known ultra-faint dwarfs. We conclude that Eri III and DELVE 1 are either the smallest dwarf galaxies yet discovered, or they are representatives of a new class of star clusters that underwent chemical evolution distinct from that of ordinary globular clusters. In the latter scenario, such objects are likely the most primordial star clusters surviving today. These possibilities can be distinguished by future measurements of carbon and/or iron abundances for larger samples of stars or improved stellar kinematics for the two systems.

==> imacs_spec_table.tex <==
\LongTables

\tabletypesize{\scriptsize}
\begin{deluxetable*}{c c c c c c c r c r c c c}
\tablecaption{IMACS Velocity and Metallicity Measurements for Eri~III and DELVE~1.\label{tab:imacs_spec_table}}

\tablehead{ID\tablenotemark{a} & RA & Dec & $g$\tablenotemark{b} & $r$\tablenotemark{b} & $z$\tablenotemark{b} & MJD & Grating & S/N & \multicolumn{1}{c}{$v$\tablenotemark{c}} & ${\rm EW}$ & ${\rm [Fe/H]}$ & Mem\tablenotemark{d} \\ 
 & (deg) & (deg) & (mag) & (mag) & (mag) &  & &  & \multicolumn{1}{c}{(\kms)} & (\AA) &  &  }
\startdata
       4745738789619969920  &   35.64276  & $ -52.37503 $ &  19.40  &  18.69  &  18.36  &  58882.1  &  G1200  &   21.2  &   \phs$65.6 \pm 1.3$  &         ...       &         ...        &  0 \\
                            &   35.64276  & $ -52.37503 $ &  19.40  &  18.69  &  18.36  &  59201.2  &  G1200  &   18.2  &   \phs$61.4 \pm 1.3$  &         ...       &         ...        &  0 \\
       4745740404527671936  &   35.65076  & $ -52.27298 $ &  17.39  &  17.30  &  17.41  &  59471.0  &   G600  &  121.7  &   \phs$64.8 \pm 3.0$  &         ...       &         ...        &  0 \\
       4745743664406724608  &   35.65818  & $ -52.20604 $ &  20.93  &  20.46  &  20.26  &  58882.1  &  G1200  &    4.2  &  \phs$151.6 \pm 4.3$  &         ...       &         ...        &  0 \\
DES\,J022238.52$-$521748.8  &   35.66050  & $ -52.29690 $ &  21.64  &  21.01  &  20.72  &  59471.0  &   G600  &    4.9  &           $z = 0.18$  &         ...       &         ...        &  0 \\
       4745740129649765504  &   35.67243  & $ -52.31168 $ &  17.87  &  17.58  &  17.50  &  59471.0  &   G600  &  109.2  &   \phs$96.5 \pm 3.0$  &         ...       &         ...        &  0 \\
DES\,J022243.71$-$521715.0  &   35.68215  & $ -52.28751 $ &  21.74  &  21.28  &  21.02  &  59471.0  &   G600  &    9.2  &   \phs$47.3 \pm 5.8$  &  $1.22 \pm 0.47$  &  $-3.02 \pm 0.44$  &  1 \\
DES\,J022243.82$-$521655.9  &   35.68260  & $ -52.28219 $ &  22.38  &  21.93  &  21.74  &  59471.0  &   G600  &    5.4  &   \phs$60.4 \pm 8.7$  &         ...       &         ...        &  1 \\
DES\,J022244.23$-$521952.5  &   35.68429  & $ -52.33125 $ &  20.05  &  19.46  &  19.26  &  59471.0  &   G600  &   16.0  &           $z = 0.07$  &         ...       &         ...        &  0 \\
       4745740335808220800  &   35.68838  & $ -52.27641 $ &  20.32  &  20.49  &  20.66  &  58882.1  &  G1200  &    3.5  &   \phs$61.8 \pm 7.0$  &         ...       &         ...        &  1 \\
                            &   35.68838  & $ -52.27641 $ &  20.32  &  20.49  &  20.66  &  59471.0  &   G600  &   14.5  &   \phs$61.5 \pm 4.8$  &         ...       &         ...        &  1 \\
DES\,J022245.46$-$521706.8  &   35.68940  & $ -52.28522 $ &  22.45  &  21.96  &  21.67  &  59471.0  &   G600  &    5.2  &  \phs$40.6 \pm 10.7$  &         ...       &         ...        &  1 \\
       4745740262792353536  &   35.69377  & $ -52.28267 $ &  20.43  &  20.64  &  20.89  &  58882.1  &  G1200  &    2.9  &   \phs$63.2 \pm 6.9$  &         ...       &         ...        &  1 \\
DES\,J022247.85$-$521712.7  &   35.69939  & $ -52.28685 $ &  21.47  &  20.85  &  20.54  &  58882.1  &  G1200  &    4.3  &  \phs$254.3 \pm 5.1$  &         ...       &         ...        &  0 \\
       4745739300719663872  &   35.69964  & $ -52.33126 $ &  19.62  &  19.35  &  19.35  &  58882.1  &  G1200  &   10.8  &          $z = 1.13?$  &         ...       &         ...        &  0 \\
                            &   35.69964  & $ -52.33126 $ &  19.62  &  19.35  &  19.35  &  59201.2  &  G1200  &    8.9  &          $z = 1.13?$  &         ...       &         ...        &  0 \\
DES\,J022248.57$-$521651.5  &   35.70236  & $ -52.28099 $ &  22.25  &  21.81  &  21.57  &  59471.0  &   G600  &    5.9  &   \phs$57.4 \pm 9.3$  &         ...       &         ...        &  1 \\
       4745740262792352128  &   35.70283  & $ -52.28476 $ &  19.41  &  18.68  &  18.31  &  58882.1  &  G1200  &   23.7  &   \phs$53.1 \pm 1.1$  &  $1.46 \pm 0.51$  &  $-3.31 \pm 0.37$  &  1 \\
                            &   35.70283  & $ -52.28476 $ &  19.41  &  18.68  &  18.31  &  59201.2  &  G1200  &   16.4  &   \phs$52.9 \pm 1.2$  &  $1.56 \pm 0.50$  &  $-3.24 \pm 0.34$  &  1 \\
                            &   35.70283  & $ -52.28476 $ &  19.41  &  18.68  &  18.31  &  59471.0  &   G600  &   67.7  &   \phs$48.9 \pm 3.1$  &  $1.42 \pm 0.21$  &  $-3.34 \pm 0.17$  &  1 \\
DES\,J022248.67$-$521540.9  &   35.70277  & $ -52.26137 $ &  22.07  &  21.70  &  21.54  &  59471.0  &   G600  &    6.5  &   \phs$74.6 \pm 7.4$  &         ...       &         ...        &  0 \\
DES\,J022248.90$-$521625.9  &   35.70375  & $ -52.27386 $ &  22.30  &  21.82  &  21.60  &  59471.0  &   G600  &    6.0  &   \phs$47.4 \pm 7.0$  &         ...       &         ...        &  1 \\
DES\,J022248.95$-$521746.0  &   35.70397  & $ -52.29610 $ &  21.27  &  20.78  &  20.62  &  59471.0  &   G600  &    6.5  &           $z = 0.05$  &         ...       &         ...        &  0 \\
       4745739030138138624  &   35.71388  & $ -52.35679 $ &  17.60  &  16.45  &  15.85  &  58882.1  &  G1200  &   93.5  &   \phs$18.9 \pm 1.0$  &         ...       &         ...        &  0 \\
                            &   35.71388  & $ -52.35679 $ &  17.60  &  16.45  &  15.85  &  59201.2  &  G1200  &   70.3  &   \phs$18.8 \pm 1.0$  &         ...       &         ...        &  0 \\
       4745691334524876032  &   35.72049  & $ -52.42902 $ &  18.35  &  17.53  &  17.14  &  58882.1  &  G1200  &   32.5  &   \phs$19.0 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &   35.72049  & $ -52.42902 $ &  18.35  &  17.53  &  17.14  &  59201.2  &  G1200  &   31.0  &   \phs$18.3 \pm 1.1$  &         ...       &         ...        &  0 \\
       4745739438158625408  &   35.73479  & $ -52.30365 $ &  20.71  &  20.13  &  20.05  &  58882.1  &  G1200  &    7.8  &           $z = 1.37$  &         ...       &         ...        &  0 \\
                            &   35.73479  & $ -52.30365 $ &  20.71  &  20.13  &  20.05  &  59201.2  &  G1200  &    5.9  &           $z = 1.37$  &         ...       &         ...        &  0 \\
       4745739476814845312  &   35.74464  & $ -52.29642 $ &  20.85  &  20.50  &  20.39  &  58882.1  &  G1200  &    4.9  &   \phs$45.8 \pm 3.2$  &         ...       &         ...        &  0 \\
       4745692056079397760  &   35.74553  & $ -52.36785 $ &  19.97  &  19.23  &  18.81  &  58882.1  &  G1200  &   14.3  &  \phs$109.5 \pm 2.3$  &         ...       &         ...        &  0 \\
                            &   35.74553  & $ -52.36785 $ &  19.97  &  19.23  &  18.81  &  59201.2  &  G1200  &   12.6  &  \phs$105.5 \pm 1.4$  &         ...       &         ...        &  0 \\
DES\,J022300.63$-$521437.1  &   35.75261  & $ -52.24363 $ &  22.89  &  22.27  &  21.69  &  59471.0  &   G600  &    4.2  &         $z \ge 1.34$  &         ...       &         ...        &  0 \\
DES\,J022301.26$-$521513.1  &   35.75525  & $ -52.25363 $ &  22.06  &  21.42  &  21.06  &  59471.0  &   G600  &    9.2  &      $-11.6 \pm 5.0$  &         ...       &         ...        &  0 \\
DES\,J022314.77$-$521241.8  &   35.81155  & $ -52.21162 $ &  22.32  &  21.90  &  21.69  &  59471.0  &   G600  &    5.5  &  \phs$14.9 \pm 10.0$  &         ...       &         ...        &  0 \\
DES\,J022318.35$-$521602.0  &   35.82645  & $ -52.26722 $ &  22.23  &  21.69  &  21.30  &  59471.0  &   G600  &    4.0  &           $z = 0.34$  &         ...       &         ...        &  0 \\
DES\,J022335.24$-$521309.7  &   35.89685  & $ -52.21937 $ &  20.99  &  20.56  &  20.41  &  59471.0  &   G600  &    7.1  &           $z = 0.06$  &         ...       &         ...        &  0 \\
DES\,J022337.43$-$521318.3  &   35.90597  & $ -52.22176 $ &  21.35  &  20.94  &  20.78  &  59471.0  &   G600  &   11.4  &  \phs$339.5 \pm 4.5$  &         ...       &         ...        &  0 \\
DES\,J022337.57$-$521043.2  &   35.90654  & $ -52.17866 $ &  21.79  &  21.35  &  21.09  &  59471.0  &   G600  &    4.8  &           $z = 0.11$  &         ...       &         ...        &  0 \\
       4745700405495864064  &   35.96694  & $ -52.21886 $ &  20.23  &  19.84  &  19.68  &  59471.0  &   G600  &   24.1  &  \phs$172.8 \pm 3.6$  &         ...       &         ...        &  0 \\
\hline
       4359353636068388224  &  247.63977  & $  -0.99505 $ &  21.87  &  20.49  &  19.61  &  59384.2  &  G1200  &    5.2  &   \phs$32.0 \pm 4.3$  &         ...       &         ...        &  0 \\
                            &  247.63977  & $  -0.99505 $ &  21.87  &  20.49  &  19.61  &  60030.0  &  G1200  &    7.1  &   \phs$31.2 \pm 4.4$  &         ...       &         ...        &  0 \\
       4359352772778121216  &  247.65121  & $  -1.02128 $ &  21.40  &  20.66  &  20.26  &  60030.0  &  G1200  &    4.2  &   \phs$98.6 \pm 5.0$  &         ...       &         ...        &  0 \\
       4359352983233361408  &  247.65709  & $  -0.99075 $ &  20.17  &  19.53  &  19.26  &  59384.2  &  G1200  &    8.1  &       $-2.8 \pm 2.3$  &         ...       &         ...        &  0 \\
                            &  247.65709  & $  -0.99075 $ &  20.17  &  19.53  &  19.26  &  59393.2  &  G1200  &    6.4  &       $-5.1 \pm 2.4$  &         ...       &         ...        &  0 \\
                            &  247.65709  & $  -0.99075 $ &  20.17  &  19.53  &  19.26  &  60030.0  &  G1200  &   10.3  &       $-1.1 \pm 1.6$  &         ...       &         ...        &  0 \\
       4359352570916497152  &  247.65965  & $  -1.03059 $ &  18.27  &  17.67  &  17.39  &  59384.2  &  G1200  &   35.1  &  \phs$132.0 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.65965  & $  -1.03059 $ &  18.27  &  17.67  &  17.39  &  59393.2  &  G1200  &   30.1  &  \phs$129.2 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.65965  & $  -1.03059 $ &  18.27  &  17.67  &  17.39  &  59751.1  &  G1200  &    7.3  &  \phs$133.6 \pm 1.9$  &         ...       &         ...        &  0 \\
                            &  247.65965  & $  -1.03059 $ &  18.27  &  17.67  &  17.39  &  60030.0  &  G1200  &   42.4  &  \phs$143.7 \pm 1.0$  &         ...       &         ...        &  0 \\
       4359354456405335552  &  247.66236  & $  -0.92961 $ &  21.34  &  19.96  &  18.92  &  59384.2  &  G1200  &   10.6  &   \phs$56.7 \pm 2.7$  &         ...       &         ...        &  0 \\
                            &  247.66236  & $  -0.92961 $ &  21.34  &  19.96  &  18.92  &  59393.2  &  G1200  &    8.3  &   \phs$62.4 \pm 3.2$  &         ...       &         ...        &  0 \\
                            &  247.66236  & $  -0.92961 $ &  21.34  &  19.96  &  18.92  &  60030.0  &  G1200  &   14.3  &   \phs$58.3 \pm 1.4$  &         ...       &         ...        &  0 \\
       4359359614662548096  &  247.67239  & $  -0.82920 $ &  17.51  &  17.07  &  16.90  &  59384.2  &  G1200  &   37.7  &      $-97.5 \pm 1.2$  &         ...       &         ...        &  0 \\
                            &  247.67239  & $  -0.82920 $ &  17.51  &  17.07  &  16.90  &  59393.2  &  G1200  &   35.3  &      $-98.5 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.67239  & $  -0.82920 $ &  17.51  &  17.07  &  16.90  &  59751.1  &  G1200  &   11.7  &      $-96.1 \pm 2.4$  &         ...       &         ...        &  0 \\
                            &  247.67239  & $  -0.82920 $ &  17.51  &  17.07  &  16.90  &  60030.0  &  G1200  &   54.0  &     $-100.2 \pm 1.0$  &         ...       &         ...        &  0 \\
       4359359099266818176  &  247.67337  & $  -0.88532 $ &  20.49  &  19.92  &  19.65  &  59384.2  &  G1200  &    5.1  &  \phs$107.6 \pm 5.1$  &         ...       &         ...        &  0 \\
                            &  247.67337  & $  -0.88532 $ &  20.49  &  19.92  &  19.65  &  59393.2  &  G1200  &    4.7  &  \phs$101.3 \pm 8.8$  &         ...       &         ...        &  0 \\
                            &  247.67337  & $  -0.88532 $ &  20.49  &  19.92  &  19.65  &  60030.0  &  G1200  &    8.1  &  \phs$109.0 \pm 3.4$  &         ...       &         ...        &  0 \\
       4359359099266817792  &  247.67414  & $  -0.88817 $ &  17.93  &  17.34  &  17.09  &  59384.2  &  G1200  &   36.4  &     $-103.4 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.67414  & $  -0.88817 $ &  17.93  &  17.34  &  17.09  &  59393.2  &  G1200  &   33.8  &     $-104.0 \pm 1.2$  &         ...       &         ...        &  0 \\
                            &  247.67414  & $  -0.88817 $ &  17.93  &  17.34  &  17.09  &  59751.1  &  G1200  &   10.1  &     $-101.7 \pm 2.3$  &         ...       &         ...        &  0 \\
                            &  247.67414  & $  -0.88817 $ &  17.93  &  17.34  &  17.09  &  60030.0  &  G1200  &   51.3  &     $-106.6 \pm 1.0$  &         ...       &         ...        &  0 \\
       4359352708355454720  &  247.68292  & $  -1.00810 $ &  20.09  &  19.52  &  19.24  &  59384.2  &  G1200  &    8.9  &   \phs$83.9 \pm 4.1$  &         ...       &         ...        &  0 \\
                            &  247.68292  & $  -1.00810 $ &  20.09  &  19.52  &  19.24  &  59393.2  &  G1200  &    7.2  &   \phs$80.4 \pm 2.3$  &         ...       &         ...        &  0 \\
                            &  247.68292  & $  -1.00810 $ &  20.09  &  19.52  &  19.24  &  60030.0  &  G1200  &   11.8  &   \phs$82.0 \pm 1.8$  &         ...       &         ...        &  0 \\
       4359356075609839872  &  247.68774  & $  -0.90517 $ &  17.92  &  17.25  &  16.90  &  59384.2  &  G1200  &   44.9  &   \phs$41.4 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.68774  & $  -0.90517 $ &  17.92  &  17.25  &  16.90  &  59393.2  &  G1200  &   40.6  &   \phs$41.3 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.68774  & $  -0.90517 $ &  17.92  &  17.25  &  16.90  &  59751.1  &  G1200  &   11.9  &   \phs$41.0 \pm 1.8$  &         ...       &         ...        &  0 \\
                            &  247.68774  & $  -0.90517 $ &  17.92  &  17.25  &  16.90  &  60030.0  &  G1200  &   60.8  &   \phs$41.8 \pm 1.0$  &         ...       &         ...        &  0 \\
       4359359923900187904  &  247.68846  & $  -0.82924 $ &  20.48  &  19.99  &  19.75  &  60030.0  &  G1200  &    6.7  &      $-99.3 \pm 3.7$  &         ...       &         ...        &  0 \\
       4359359923900185088  &  247.69159  & $  -0.83165 $ &  19.49  &  18.34  &  17.60  &  59384.2  &  G1200  &   24.9  &       $-8.0 \pm 1.4$  &         ...       &         ...        &  0 \\
                            &  247.69159  & $  -0.83165 $ &  19.49  &  18.34  &  17.60  &  59393.2  &  G1200  &   22.5  &    \phs$7.1 \pm 2.4$  &         ...       &         ...        &  0 \\
                            &  247.69159  & $  -0.83165 $ &  19.49  &  18.34  &  17.60  &  59751.1  &  G1200  &    6.8  &      $-16.9 \pm 8.1$  &         ...       &         ...        &  0 \\
                            &  247.69159  & $  -0.83165 $ &  19.49  &  18.34  &  17.60  &  60030.0  &  G1200  &   35.7  &      $-18.0 \pm 1.2$  &         ...       &         ...        &  0 \\
       4359352639635977344  &  247.69382  & $  -1.01965 $ &  19.50  &  18.80  &  18.40  &  59384.2  &  G1200  &   18.0  &   \phs$68.4 \pm 1.6$  &         ...       &         ...        &  0 \\
                            &  247.69382  & $  -1.01965 $ &  19.50  &  18.80  &  18.40  &  59393.2  &  G1200  &   14.6  &   \phs$64.5 \pm 1.4$  &         ...       &         ...        &  0 \\
                            &  247.69382  & $  -1.01965 $ &  19.50  &  18.80  &  18.40  &  60030.0  &  G1200  &   21.8  &   \phs$65.7 \pm 1.2$  &         ...       &         ...        &  0 \\
       4359356178689761280  &  247.69831  & $  -0.88173 $ &  17.29  &  16.54  &  16.10  &  59384.2  &  G1200  &   66.4  &   \phs$18.6 \pm 1.0$  &         ...       &         ...        &  0 \\
                            &  247.69831  & $  -0.88173 $ &  17.29  &  16.54  &  16.10  &  59393.2  &  G1200  &   60.7  &   \phs$18.2 \pm 1.0$  &         ...       &         ...        &  0 \\
                            &  247.69831  & $  -0.88173 $ &  17.29  &  16.54  &  16.10  &  59751.1  &  G1200  &   21.2  &   \phs$17.2 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.69831  & $  -0.88173 $ &  17.29  &  16.54  &  16.10  &  60030.0  &  G1200  &   90.4  &   \phs$18.2 \pm 1.0$  &         ...       &         ...        &  0 \\
       4359356174395853824  &  247.69951  & $  -0.88651 $ &  20.66  &  20.25  &  20.09  &  60030.0  &  G1200  &    5.7  &     $-240.6 \pm 2.4$  &         ...       &         ...        &  0 \\
       4359353356899458432  &  247.70262  & $  -0.96713 $ &  21.24  &  20.04  &  19.38  &  59384.2  &  G1200  &    7.9  &  \phs$129.0 \pm 5.8$  &         ...       &         ...        &  0 \\
                            &  247.70262  & $  -0.96713 $ &  21.24  &  20.04  &  19.38  &  59393.2  &  G1200  &    6.1  &  \phs$126.5 \pm 4.2$  &         ...       &         ...        &  0 \\
                            &  247.70262  & $  -0.96713 $ &  21.24  &  20.04  &  19.38  &  60030.0  &  G1200  &   10.7  &  \phs$123.0 \pm 1.7$  &         ...       &         ...        &  0 \\
       4359164794946409088  &  247.70392  & $  -1.04361 $ &  19.47  &  18.89  &  18.63  &  59384.2  &  G1200  &   15.5  &   \phs$67.9 \pm 1.9$  &         ...       &         ...        &  0 \\
                            &  247.70392  & $  -1.04361 $ &  19.47  &  18.89  &  18.63  &  59393.2  &  G1200  &   12.6  &   \phs$68.9 \pm 1.7$  &         ...       &         ...        &  0 \\
                            &  247.70392  & $  -1.04361 $ &  19.47  &  18.89  &  18.63  &  60030.0  &  G1200  &   18.0  &   \phs$67.2 \pm 1.3$  &         ...       &         ...        &  0 \\
       4359353361190494336  &  247.70497  & $  -0.97204 $ &  21.06  &  20.58  &  20.44  &  60030.0  &  G1200  &    4.2  &     $-248.8 \pm 3.5$  &         ...       &         ...        &  0 \\
       4359359923900179072  &  247.70653  & $  -0.83140 $ &  19.59  &  19.02  &  18.72  &  59384.2  &  G1200  &   11.6  &     $-112.1 \pm 1.6$  &         ...       &         ...        &  0 \\
                            &  247.70653  & $  -0.83140 $ &  19.59  &  19.02  &  18.72  &  59393.2  &  G1200  &   10.2  &     $-110.9 \pm 2.6$  &         ...       &         ...        &  0 \\
                            &  247.70653  & $  -0.83140 $ &  19.59  &  19.02  &  18.72  &  60030.0  &  G1200  &   17.5  &     $-115.7 \pm 1.2$  &         ...       &         ...        &  0 \\
       4359355865154616704  &  247.70840  & $  -0.91167 $ &  19.83  &  19.22  &  18.92  &  59384.2  &  G1200  &   11.3  &   \phs$39.5 \pm 2.1$  &         ...       &         ...        &  0 \\
                            &  247.70840  & $  -0.91167 $ &  19.83  &  19.22  &  18.92  &  59393.2  &  G1200  &    9.8  &   \phs$43.1 \pm 2.5$  &         ...       &         ...        &  0 \\
                            &  247.70840  & $  -0.91167 $ &  19.83  &  19.22  &  18.92  &  60030.0  &  G1200  &   16.7  &   \phs$42.2 \pm 1.3$  &         ...       &         ...        &  0 \\
       4359359958259917952  &  247.70882  & $  -0.82880 $ &  20.12  &  19.61  &  19.38  &  59384.2  &  G1200  &    6.4  &      $-21.4 \pm 3.5$  &         ...       &         ...        &  0 \\
                            &  247.70882  & $  -0.82880 $ &  20.12  &  19.61  &  19.38  &  59393.2  &  G1200  &    5.9  &      $-25.0 \pm 3.0$  &         ...       &         ...        &  0 \\
                            &  247.70882  & $  -0.82880 $ &  20.12  &  19.61  &  19.38  &  60030.0  &  G1200  &   10.2  &      $-19.9 \pm 1.8$  &         ...       &         ...        &  0 \\
       4359353356893691776  &  247.71368  & $  -0.96735 $ &  19.60  &  19.02  &  18.70  &  59384.2  &  G1200  &   14.0  &     $-403.8 \pm 1.5$  &  $2.18 \pm 0.34$  &  $-2.25 \pm 0.20$  &  1 \\
                            &  247.71368  & $  -0.96735 $ &  19.60  &  19.02  &  18.70  &  59393.2  &  G1200  &   11.6  &     $-403.1 \pm 1.7$  &  $1.44 \pm 0.59$  &  $-2.73 \pm 0.47$  &  1 \\
                            &  247.71368  & $  -0.96735 $ &  19.60  &  19.02  &  18.70  &  60030.0  &  G1200  &   19.9  &     $-402.0 \pm 1.2$  &  $1.93 \pm 0.42$  &  $-2.40 \pm 0.26$  &  1 \\
       4359353155032064256  &  247.71490  & $  -0.97875 $ &  21.02  &  20.69  &  20.61  &  60030.0  &  G1200  &    3.8  &     $-399.7 \pm 3.7$  &         ...       &         ...        &  1 \\
       4359355800731933312  &  247.71505  & $  -0.92495 $ &  18.47  &  17.77  &  17.46  &  59384.2  &  G1200  &   30.7  &   \phs$31.7 \pm 1.2$  &         ...       &         ...        &  0 \\
                            &  247.71505  & $  -0.92495 $ &  18.47  &  17.77  &  17.46  &  59393.2  &  G1200  &   27.4  &   \phs$31.9 \pm 1.7$  &         ...       &         ...        &  0 \\
                            &  247.71505  & $  -0.92495 $ &  18.47  &  17.77  &  17.46  &  59751.1  &  G1200  &    7.9  &   \phs$29.3 \pm 2.5$  &         ...       &         ...        &  0 \\
                            &  247.71505  & $  -0.92495 $ &  18.47  &  17.77  &  17.46  &  60030.0  &  G1200  &   44.0  &   \phs$30.9 \pm 1.1$  &         ...       &         ...        &  0 \\
       4359165001104849792  &  247.71745  & $  -1.01887 $ &  20.00  &  19.30  &  18.96  &  59384.2  &  G1200  &   11.5  &      $-24.3 \pm 1.8$  &         ...       &         ...        &  0 \\
                            &  247.71745  & $  -1.01887 $ &  20.00  &  19.30  &  18.96  &  59393.2  &  G1200  &    9.0  &      $-24.9 \pm 2.4$  &         ...       &         ...        &  0 \\
                            &  247.71745  & $  -1.01887 $ &  20.00  &  19.30  &  18.96  &  60030.0  &  G1200  &   13.5  &      $-22.7 \pm 1.5$  &         ...       &         ...        &  0 \\
       4359356213048800128  &  247.71795  & $  -0.88796 $ &  20.84  &  20.51  &  20.33  &  60030.0  &  G1200  &    4.9  &     $-398.9 \pm 3.1$  &         ...       &         ...        &  1 \\
       4359353150735257472  &  247.71988  & $  -0.97731 $ &  20.36  &  19.90  &  19.68  &  59384.2  &  G1200  &    6.0  &     $-403.4 \pm 3.4$  &         ...       &         ...        &  1 \\
                            &  247.71988  & $  -0.97731 $ &  20.36  &  19.90  &  19.68  &  59393.2  &  G1200  &    4.8  &     $-404.7 \pm 3.0$  &         ...       &         ...        &  1 \\
                            &  247.71988  & $  -0.97731 $ &  20.36  &  19.90  &  19.68  &  60030.0  &  G1200  &    8.7  &     $-400.8 \pm 2.2$  &         ...       &         ...        &  1 \\
       4359356213048404608  &  247.72113  & $  -0.88161 $ &  18.86  &  18.29  &  17.98  &  59384.2  &  G1200  &   21.7  &     $-131.9 \pm 1.3$  &         ...       &         ...        &  0 \\
                            &  247.72113  & $  -0.88161 $ &  18.86  &  18.29  &  17.98  &  59393.2  &  G1200  &   19.5  &     $-129.2 \pm 1.4$  &         ...       &         ...        &  0 \\
                            &  247.72113  & $  -0.88161 $ &  18.86  &  18.29  &  17.98  &  59751.1  &  G1200  &    4.9  &     $-123.8 \pm 4.1$  &         ...       &         ...        &  0 \\
                            &  247.72113  & $  -0.88161 $ &  18.86  &  18.29  &  17.98  &  60030.0  &  G1200  &   31.2  &     $-131.7 \pm 1.1$  &         ...       &         ...        &  0 \\
       4359353155032064640  &  247.72368  & $  -0.98238 $ &  20.55  &  20.16  &  20.03  &  59384.2  &  G1200  &    4.6  &     $-403.5 \pm 4.3$  &         ...       &         ...        &  1 \\
                            &  247.72368  & $  -0.98238 $ &  20.55  &  20.16  &  20.03  &  60030.0  &  G1200  &    6.3  &     $-397.7 \pm 3.9$  &         ...       &         ...        &  1 \\
       4359353253820330624  &  247.72520  & $  -0.96842 $ &  20.72  &  20.30  &  20.12  &  59384.2  &  G1200  &    4.3  &     $-404.2 \pm 4.2$  &         ...       &         ...        &  1 \\
                            &  247.72520  & $  -0.96842 $ &  20.72  &  20.30  &  20.12  &  60030.0  &  G1200  &    6.1  &     $-405.6 \pm 2.8$  &         ...       &         ...        &  1 \\
       4359353258111283328  &  247.72604  & $  -0.96706 $ &  16.70  &  15.97  &  15.63  &  59384.2  &  G1200  &   96.3  &     $-403.2 \pm 1.0$  &  $2.53 \pm 0.20$  &  $-2.69 \pm 0.11$  &  1 \\
                            &  247.72604  & $  -0.96706 $ &  16.70  &  15.97  &  15.63  &  59393.2  &  G1200  &   84.8  &     $-403.0 \pm 1.0$  &  $2.28 \pm 0.21$  &  $-2.80 \pm 0.12$  &  1 \\
                            &  247.72604  & $  -0.96706 $ &  16.70  &  15.97  &  15.63  &  59751.1  &  G1200  &   30.1  &     $-401.9 \pm 1.1$  &  $1.90 \pm 0.32$  &  $-3.00 \pm 0.19$  &  1 \\
                            &  247.72604  & $  -0.96706 $ &  16.70  &  15.97  &  15.63  &  60030.0  &  G1200  &  126.7  &     $-403.1 \pm 1.0$  &  $2.20 \pm 0.21$  &  $-2.84 \pm 0.12$  &  1 \\
       4359356247408141184  &  247.72774  & $  -0.87931 $ &  18.76  &  17.92  &  17.51  &  59384.2  &  G1200  &   28.6  &      $-29.7 \pm 1.2$  &         ...       &         ...        &  0 \\
                            &  247.72774  & $  -0.87931 $ &  18.76  &  17.92  &  17.51  &  59393.2  &  G1200  &   25.7  &      $-29.4 \pm 1.2$  &         ...       &         ...        &  0 \\
                            &  247.72774  & $  -0.87931 $ &  18.76  &  17.92  &  17.51  &  59751.1  &  G1200  &    7.6  &      $-32.5 \pm 2.1$  &         ...       &         ...        &  0 \\
                            &  247.72774  & $  -0.87931 $ &  18.76  &  17.92  &  17.51  &  60030.0  &  G1200  &   41.1  &      $-31.0 \pm 1.1$  &         ...       &         ...        &  0 \\
       4359164691867194624  &  247.72827  & $  -1.05160 $ &  19.93  &  19.24  &  18.89  &  59384.2  &  G1200  &   13.0  &      $-85.1 \pm 1.9$  &         ...       &         ...        &  0 \\
                            &  247.72827  & $  -1.05160 $ &  19.93  &  19.24  &  18.89  &  59393.2  &  G1200  &   10.3  &      $-85.8 \pm 2.7$  &         ...       &         ...        &  0 \\
                            &  247.72827  & $  -1.05160 $ &  19.93  &  19.24  &  18.89  &  60030.0  &  G1200  &   13.8  &      $-84.2 \pm 2.1$  &         ...       &         ...        &  0 \\
       4359353086312587776  &  247.73025  & $  -0.98792 $ &  18.27  &  17.62  &  17.31  &  59384.2  &  G1200  &   38.1  &      $-79.0 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.73025  & $  -0.98792 $ &  18.27  &  17.62  &  17.31  &  59393.2  &  G1200  &   32.6  &      $-78.4 \pm 1.3$  &         ...       &         ...        &  0 \\
                            &  247.73025  & $  -0.98792 $ &  18.27  &  17.62  &  17.31  &  59751.1  &  G1200  &    8.6  &      $-77.6 \pm 3.1$  &         ...       &         ...        &  0 \\
                            &  247.73025  & $  -0.98792 $ &  18.27  &  17.62  &  17.31  &  60030.0  &  G1200  &   49.5  &      $-80.9 \pm 1.1$  &         ...       &         ...        &  0 \\
       4359354976098213248  &  247.74093  & $  -0.94068 $ &  21.13  &  20.79  &  20.61  &  60030.0  &  G1200  &    3.9  &     $-406.7 \pm 4.1$  &         ...       &         ...        &  1 \\
       4359356041248190976  &  247.74149  & $  -0.87822 $ &  20.78  &  20.36  &  20.13  &  60030.0  &  G1200  &    4.3  &      $-45.6 \pm 6.7$  &         ...       &         ...        &  0 \\
       4359165104184057984  &  247.74396  & $  -1.02724 $ &  19.56  &  19.13  &  18.92  &  59384.2  &  G1200  &   13.3  &      $-69.6 \pm 1.8$  &         ...       &         ...        &  0 \\
                            &  247.74396  & $  -1.02724 $ &  19.56  &  19.13  &  18.92  &  59393.2  &  G1200  &   10.6  &      $-70.5 \pm 2.0$  &         ...       &         ...        &  0 \\
                            &  247.74396  & $  -1.02724 $ &  19.56  &  19.13  &  18.92  &  60030.0  &  G1200  &   15.1  &      $-68.8 \pm 1.5$  &         ...       &         ...        &  0 \\
       4359359889540433536  &  247.74595  & $  -0.81389 $ &  19.10  &  18.35  &  17.93  &  59384.2  &  G1200  &   21.2  &       $-0.3 \pm 1.2$  &         ...       &         ...        &  0 \\
                            &  247.74595  & $  -0.81389 $ &  19.10  &  18.35  &  17.93  &  59393.2  &  G1200  &   18.8  &       $-1.1 \pm 1.2$  &         ...       &         ...        &  0 \\
                            &  247.74595  & $  -0.81389 $ &  19.10  &  18.35  &  17.93  &  59751.1  &  G1200  &    5.3  &       $-0.4 \pm 2.3$  &         ...       &         ...        &  0 \\
                            &  247.74595  & $  -0.81389 $ &  19.10  &  18.35  &  17.93  &  60030.0  &  G1200  &   30.0  &    \phs$2.5 \pm 1.1$  &         ...       &         ...        &  0 \\
       4359355938170475648  &  247.74622  & $  -0.90659 $ &  17.47  &  16.83  &  16.48  &  59384.2  &  G1200  &   55.5  &       $-5.3 \pm 1.0$  &         ...       &         ...        &  0 \\
                            &  247.74622  & $  -0.90659 $ &  17.47  &  16.83  &  16.48  &  59393.2  &  G1200  &   49.7  &       $-4.3 \pm 1.0$  &         ...       &         ...        &  0 \\
                            &  247.74622  & $  -0.90659 $ &  17.47  &  16.83  &  16.48  &  59751.1  &  G1200  &   16.5  &       $-7.4 \pm 1.3$  &         ...       &         ...        &  0 \\
                            &  247.74622  & $  -0.90659 $ &  17.47  &  16.83  &  16.48  &  60030.0  &  G1200  &   77.6  &       $-5.4 \pm 1.0$  &         ...       &         ...        &  0 \\
       4359164726226935424  &  247.74679  & $  -1.03375 $ &  18.26  &  17.64  &  17.36  &  59384.2  &  G1200  &   38.0  &       $-4.6 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.74679  & $  -1.03375 $ &  18.26  &  17.64  &  17.36  &  59393.2  &  G1200  &   32.4  &       $-5.3 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.74679  & $  -1.03375 $ &  18.26  &  17.64  &  17.36  &  59751.1  &  G1200  &    8.3  &       $-3.1 \pm 1.9$  &         ...       &         ...        &  0 \\
                            &  247.74679  & $  -1.03375 $ &  18.26  &  17.64  &  17.36  &  60030.0  &  G1200  &   46.3  &       $-3.6 \pm 1.0$  &         ...       &         ...        &  0 \\
       4359165344702228480  &  247.74956  & $  -1.00258 $ &  18.52  &  17.84  &  17.48  &  59384.2  &  G1200  &   35.1  &      $-26.2 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.74956  & $  -1.00258 $ &  18.52  &  17.84  &  17.48  &  59393.2  &  G1200  &   29.6  &      $-25.8 \pm 1.2$  &         ...       &         ...        &  0 \\
                            &  247.74956  & $  -1.00258 $ &  18.52  &  17.84  &  17.48  &  59751.1  &  G1200  &    7.8  &      $-27.2 \pm 2.3$  &         ...       &         ...        &  0 \\
                            &  247.74956  & $  -1.00258 $ &  18.52  &  17.84  &  17.48  &  60030.0  &  G1200  &   43.7  &      $-26.9 \pm 1.1$  &         ...       &         ...        &  0 \\
       4359165344702227840  &  247.75024  & $  -1.01005 $ &  19.47  &  18.80  &  18.47  &  59384.2  &  G1200  &   17.9  &      $-14.8 \pm 1.7$  &         ...       &         ...        &  0 \\
                            &  247.75024  & $  -1.01005 $ &  19.47  &  18.80  &  18.47  &  59393.2  &  G1200  &   14.8  &      $-13.9 \pm 1.5$  &         ...       &         ...        &  0 \\
                            &  247.75024  & $  -1.01005 $ &  19.47  &  18.80  &  18.47  &  60030.0  &  G1200  &   22.8  &      $-12.9 \pm 1.3$  &         ...       &         ...        &  0 \\
       4359356659725001088  &  247.75076  & $  -0.86125 $ &  18.11  &  17.65  &  17.47  &  59384.2  &  G1200  &   30.5  &      $-84.7 \pm 1.2$  &         ...       &         ...        &  0 \\
                            &  247.75076  & $  -0.86125 $ &  18.11  &  17.65  &  17.47  &  59393.2  &  G1200  &   27.1  &      $-85.1 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.75076  & $  -0.86125 $ &  18.11  &  17.65  &  17.47  &  59751.1  &  G1200  &    8.3  &      $-81.8 \pm 2.2$  &         ...       &         ...        &  0 \\
                            &  247.75076  & $  -0.86125 $ &  18.11  &  17.65  &  17.47  &  60030.0  &  G1200  &   43.9  &      $-84.0 \pm 1.1$  &         ...       &         ...        &  0 \\
       4359356659725002496  &  247.75313  & $  -0.85683 $ &  18.09  &  17.54  &  17.32  &  59384.2  &  G1200  &   33.6  &      $-22.9 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.75313  & $  -0.85683 $ &  18.09  &  17.54  &  17.32  &  59393.2  &  G1200  &   29.8  &      $-23.4 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.75313  & $  -0.85683 $ &  18.09  &  17.54  &  17.32  &  59751.1  &  G1200  &    8.9  &     $-445.5 \pm 7.2$  &         ...       &         ...        &  0 \\
                            &  247.75313  & $  -0.85683 $ &  18.09  &  17.54  &  17.32  &  60030.0  &  G1200  &   47.5  &      $-21.6 \pm 1.0$  &         ...       &         ...        &  0 \\
       4359165447781444224  &  247.75471  & $  -0.99825 $ &  20.25  &  19.69  &  19.45  &  59384.2  &  G1200  &    8.1  &     $-139.4 \pm 2.7$  &         ...       &         ...        &  0 \\
                            &  247.75471  & $  -0.99825 $ &  20.25  &  19.69  &  19.45  &  59393.2  &  G1200  &    6.4  &     $-137.1 \pm 4.6$  &         ...       &         ...        &  0 \\
                            &  247.75471  & $  -0.99825 $ &  20.25  &  19.69  &  19.45  &  60030.0  &  G1200  &    9.7  &     $-133.4 \pm 3.1$  &         ...       &         ...        &  0 \\
       4359355972530216832  &  247.75736  & $  -0.89262 $ &  18.06  &  17.46  &  17.18  &  59384.2  &  G1200  &   38.9  &      $-42.4 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.75736  & $  -0.89262 $ &  18.06  &  17.46  &  17.18  &  59393.2  &  G1200  &   34.1  &      $-35.9 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.75736  & $  -0.89262 $ &  18.06  &  17.46  &  17.18  &  59751.1  &  G1200  &   10.1  &      $-29.2 \pm 2.5$  &         ...       &         ...        &  0 \\
                            &  247.75736  & $  -0.89262 $ &  18.06  &  17.46  &  17.18  &  60030.0  &  G1200  &   54.1  &      $-40.1 \pm 1.0$  &         ...       &         ...        &  0 \\
       4359165344702228864  &  247.75781  & $  -1.00256 $ &  18.38  &  17.81  &  17.56  &  59384.2  &  G1200  &   34.4  &   \phs$87.5 \pm 1.2$  &         ...       &         ...        &  0 \\
                            &  247.75781  & $  -1.00256 $ &  18.38  &  17.81  &  17.56  &  59393.2  &  G1200  &   29.0  &   \phs$88.4 \pm 1.2$  &         ...       &         ...        &  0 \\
                            &  247.75781  & $  -1.00256 $ &  18.38  &  17.81  &  17.56  &  59751.1  &  G1200  &    7.7  &   \phs$93.2 \pm 4.9$  &         ...       &         ...        &  0 \\
                            &  247.75781  & $  -1.00256 $ &  18.38  &  17.81  &  17.56  &  60030.0  &  G1200  &   43.4  &   \phs$89.3 \pm 1.1$  &         ...       &         ...        &  0 \\
       4359355177960351488  &  247.75826  & $  -0.91652 $ &  21.73  &  20.56  &  19.90  &  59384.2  &  G1200  &    5.1  &      $-88.2 \pm 3.1$  &         ...       &         ...        &  0 \\
                            &  247.75826  & $  -0.91652 $ &  21.73  &  20.56  &  19.90  &  59393.2  &  G1200  &    3.9  &      $-88.7 \pm 5.2$  &         ...       &         ...        &  0 \\
                            &  247.75826  & $  -0.91652 $ &  21.73  &  20.56  &  19.90  &  60030.0  &  G1200  &    7.3  &      $-85.0 \pm 3.0$  &         ...       &         ...        &  0 \\
       4359354804299081600  &  247.76217  & $  -0.94860 $ &  17.78  &  17.16  &  16.85  &  59384.2  &  G1200  &   48.6  &      $-13.1 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.76217  & $  -0.94860 $ &  17.78  &  17.16  &  16.85  &  59393.2  &  G1200  &   42.3  &      $-12.7 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.76217  & $  -0.94860 $ &  17.78  &  17.16  &  16.85  &  59751.1  &  G1200  &   12.8  &      $-11.5 \pm 1.6$  &         ...       &         ...        &  0 \\
                            &  247.76217  & $  -0.94860 $ &  17.78  &  17.16  &  16.85  &  60030.0  &  G1200  &   65.8  &      $-12.4 \pm 1.0$  &         ...       &         ...        &  0 \\
       4359356865883832192  &  247.76363  & $  -0.82832 $ &  18.19  &  17.64  &  17.39  &  59384.2  &  G1200  &   32.9  &      $-12.2 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.76363  & $  -0.82832 $ &  18.19  &  17.64  &  17.39  &  59393.2  &  G1200  &   29.4  &     $-389.5 \pm 2.3$  &         ...       &         ...        &  0 \\
                            &  247.76363  & $  -0.82832 $ &  18.19  &  17.64  &  17.39  &  59751.1  &  G1200  &    8.8  &       $-9.5 \pm 1.2$  &         ...       &         ...        &  0 \\
                            &  247.76363  & $  -0.82832 $ &  18.19  &  17.64  &  17.39  &  60030.0  &  G1200  &   45.5  &      $-11.7 \pm 1.0$  &         ...       &         ...        &  0 \\
       4359383288522252672  &  247.76829  & $  -0.81574 $ &  20.34  &  19.94  &  19.74  &  60030.0  &  G1200  &    6.4  &      $-60.1 \pm 1.1$  &         ...       &         ...        &  0 \\
       4359380333584746880  &  247.77140  & $  -0.82537 $ &  19.50  &  18.80  &  18.37  &  59384.2  &  G1200  &   14.8  &   \phs$17.0 \pm 1.5$  &         ...       &         ...        &  0 \\
                            &  247.77140  & $  -0.82537 $ &  19.50  &  18.80  &  18.37  &  59393.2  &  G1200  &   12.9  &   \phs$10.0 \pm 2.2$  &         ...       &         ...        &  0 \\
                            &  247.77140  & $  -0.82537 $ &  19.50  &  18.80  &  18.37  &  60030.0  &  G1200  &   20.8  &   \phs$18.5 \pm 1.4$  &         ...       &         ...        &  0 \\
       4359355594573090560  &  247.77338  & $  -0.88722 $ &  17.43  &  16.92  &  16.71  &  59384.2  &  G1200  &   51.3  &      $-18.7 \pm 1.0$  &         ...       &         ...        &  0 \\
                            &  247.77338  & $  -0.88722 $ &  17.43  &  16.92  &  16.71  &  59393.2  &  G1200  &   45.8  &      $-19.7 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.77338  & $  -0.88722 $ &  17.43  &  16.92  &  16.71  &  59751.1  &  G1200  &   14.7  &      $-14.9 \pm 1.6$  &         ...       &         ...        &  0 \\
                            &  247.77338  & $  -0.88722 $ &  17.43  &  16.92  &  16.71  &  60030.0  &  G1200  &   70.2  &      $-16.9 \pm 1.0$  &         ...       &         ...        &  0 \\
       4359356556645778560  &  247.77398  & $  -0.86342 $ &  18.30  &  17.79  &  17.58  &  59384.2  &  G1200  &   30.3  &      $-46.1 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.77398  & $  -0.86342 $ &  18.30  &  17.79  &  17.58  &  59393.2  &  G1200  &   26.9  &      $-47.6 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &  247.77398  & $  -0.86342 $ &  18.30  &  17.79  &  17.58  &  59751.1  &  G1200  &    7.9  &      $-15.5 \pm 8.7$  &         ...       &         ...        &  0 \\
                            &  247.77398  & $  -0.86342 $ &  18.30  &  17.79  &  17.58  &  60030.0  &  G1200  &   42.2  &      $-45.9 \pm 1.0$  &         ...       &         ...        &  0 \\
\enddata
\tablenotetext{a}{Source\_id for stars in the Gaia~DR3 catalog, and DES identifier for those that are not.}
\tablenotetext{b}{Quoted magnitudes represent the weighted-average PSF magnitude derived from the DES images using SourceExtractor \citep{drlica15}.}
\tablenotetext{c}{Heliocentric velocities are listed for stars and approximate redshifts are given for background galaxies.}
\tablenotetext{d}{A value of 1 indicates that the star is a member of the relevant satellite, whereas 0 indicates a non-member.}
\end{deluxetable*}


==> linetab_full.tex <==
\begin{deluxetable*}{lrrrrrrrrrrrrrrrrr}
\tablecolumns{17}
\tabletypesize{\footnotesize}
\tablecaption{\label{tab:lines}Line Measurements}
\tablehead{Star & $\lambda$ & ID & $\chi$ & $\log gf$ & EW & $\sigma$(EW) & FWHM & ul & $\log \epsilon_i$ & $\sigma_i$ & $e_i$ & $s_X$ & $\delta_{i,\teff}$ & $\delta_{i,\logg}$ & $\delta_{i,\nu_t}$ & $\delta_{i,\text{[M/H]}}$ }
\startdata
DELVE~1-S1 & 6300.30 &   8.0 &  0.00 & -9.69 &  15.8 &  3.2 &  0.23 &   &  7.30 &  0.20 &  0.09 &  0.10 & +0.10 & +0.10 & -0.00 & +0.01 \\
DELVE~1-S1 & 7771.94 &   8.0 &  9.15 &  0.37 &  30.6 &  3.8 &  0.27 &   &  7.76 &  0.23 &  0.09 &  0.10 & -0.13 & +0.13 & -0.01 & -0.00 \\
DELVE~1-S1 & 7774.17 &   8.0 &  9.15 &  0.22 &  17.4 &  2.9 &  0.23 &   &  7.54 &  0.23 &  0.10 &  0.10 & -0.13 & +0.13 & -0.01 & -0.00 \\
DELVE~1-S1 & 7775.39 &   8.0 &  9.15 &  0.00 &  13.5 &  2.9 &  0.30 &   &  7.61 &  0.24 &  0.12 &  0.10 & -0.12 & +0.13 & -0.00 & +0.00 \\
DELVE~1-S1 & 5889.95 &  11.0 &  0.00 &  0.11 & 150.3 &  2.8 &  0.29 &   &  3.70 &  0.24 &  0.05 &  0.10 & +0.16 & -0.04 & -0.14 & -0.02 \\
DELVE~1-S1 & 5895.92 &  11.0 &  0.00 & -0.19 & 168.9 &  5.0 &  0.34 &   &  4.31 &  0.26 &  0.08 &  0.10 & +0.17 & -0.06 & -0.14 & -0.02 \\
DELVE~1-S1 & 4702.99 &  12.0 &  4.33 & -0.44 &  57.3 &  2.5 &  0.18 &   &  5.11 &  0.13 &  0.04 &  0.10 & +0.07 & -0.02 & -0.02 & +0.00 \\
DELVE~1-S1 & 5172.68 &  12.0 &  2.71 & -0.36 & 181.8 &  5.1 &  0.27 &   &  5.24 &  0.25 &  0.06 &  0.10 & +0.16 & -0.10 & -0.11 & -0.01 \\
DELVE~1-S1 & 5183.60 &  12.0 &  2.72 & -0.17 & 196.4 &  5.7 &  0.29 &   &  5.23 &  0.25 &  0.06 &  0.10 & +0.17 & -0.11 & -0.09 & -0.01 \\
DELVE~1-S1 & 5528.40 &  12.0 &  4.35 & -0.55 &  52.9 &  3.6 &  0.23 &   &  5.15 &  0.14 &  0.06 &  0.10 & +0.08 & -0.02 & -0.02 & +0.00 \\
DELVE~1-S1 & 7698.96 &  19.0 &  0.00 & -0.18 &  27.3 &  3.8 &  0.32 &   &  2.80 &  0.17 &  0.08 &  0.10 & +0.11 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 4425.44 &  20.0 &  1.88 & -0.39 &  58.4 &  3.9 &  0.22 &   &  4.17 &  0.16 &  0.07 &  0.10 & +0.10 & -0.02 & -0.04 & +0.00 \\
DELVE~1-S1 & 4435.69 &  20.0 &  1.89 & -0.53 &  36.6 &  2.9 &  0.16 &   &  3.95 &  0.15 &  0.05 &  0.10 & +0.09 & -0.02 & -0.02 & +0.00 \\
DELVE~1-S1 & 4454.78 &  20.0 &  1.90 &  0.23 &  80.1 &  5.8 &  0.20 &   &  3.95 &  0.20 &  0.12 &  0.10 & +0.10 & -0.02 & -0.07 & -0.00 \\
DELVE~1-S1 & 4455.89 &  20.0 &  1.90 & -0.54 &  31.8 &  2.4 &  0.19 &   &  3.88 &  0.15 &  0.05 &  0.10 & +0.10 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 6102.72 &  20.0 &  1.88 & -0.82 &  21.8 &  3.3 &  0.26 &   &  3.84 &  0.16 &  0.08 &  0.10 & +0.10 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 6122.22 &  20.0 &  1.89 & -0.34 &  44.3 &  3.2 &  0.27 &   &  3.81 &  0.15 &  0.05 &  0.10 & +0.10 & -0.02 & -0.02 & +0.00 \\
DELVE~1-S1 & 6162.17 &  20.0 &  1.90 & -0.12 &  54.1 &  2.4 &  0.25 &   &  3.76 &  0.15 &  0.04 &  0.10 & +0.10 & -0.02 & -0.03 & +0.00 \\
DELVE~1-S1 & 6439.07 &  20.0 &  2.52 &  0.39 &  51.6 &  2.3 &  0.29 &   &  3.90 &  0.14 &  0.04 &  0.10 & +0.09 & -0.01 & -0.03 & +0.00 \\
DELVE~1-S1 & 4533.24 &  22.0 &  0.85 &  0.54 &  31.5 &  2.4 &  0.17 &   &  2.18 &  0.19 &  0.05 &  0.10 & +0.15 & -0.03 & -0.01 & +0.00 \\
DELVE~1-S1 & 4534.78 &  22.0 &  0.84 &  0.35 &  26.8 &  3.4 &  0.24 &   &  2.27 &  0.20 &  0.07 &  0.10 & +0.15 & -0.03 & -0.01 & +0.00 \\
DELVE~1-S1 & 5210.38 &  22.0 &  0.05 & -0.82 &  16.3 &  4.5 &  0.18 &   &  2.21 &  0.24 &  0.13 &  0.10 & +0.17 & -0.03 & -0.00 & +0.00 \\
DELVE~1-S1 & 4417.71 &  22.1 &  1.17 & -1.19 &  72.1 &  3.3 &  0.18 &   &  2.14 &  0.18 &  0.05 &  0.10 & +0.07 & +0.10 & -0.07 & +0.01 \\
DELVE~1-S1 & 4418.33 &  22.1 &  1.24 & -1.99 &  27.6 &  3.5 &  0.18 &   &  2.26 &  0.17 &  0.07 &  0.10 & +0.07 & +0.10 & -0.01 & +0.01 \\
DELVE~1-S1 & 4443.80 &  22.1 &  1.08 & -0.71 &  99.0 &  2.2 &  0.17 &   &  2.09 &  0.21 &  0.05 &  0.10 & +0.08 & +0.10 & -0.13 & +0.00 \\
DELVE~1-S1 & 4444.55 &  22.1 &  1.12 & -2.20 &  23.9 &  3.2 &  0.16 &   &  2.24 &  0.17 &  0.07 &  0.10 & +0.07 & +0.10 & -0.01 & +0.01 \\
DELVE~1-S1 & 4450.48 &  22.1 &  1.08 & -1.52 &  59.0 &  3.0 &  0.17 &   &  2.14 &  0.17 &  0.05 &  0.10 & +0.07 & +0.10 & -0.04 & +0.01 \\
DELVE~1-S1 & 4464.45 &  22.1 &  1.16 & -1.81 &  40.4 &  3.1 &  0.18 &   &  2.21 &  0.17 &  0.05 &  0.10 & +0.07 & +0.10 & -0.02 & +0.01 \\
DELVE~1-S1 & 4470.85 &  22.1 &  1.17 & -2.02 &  16.8 &  3.7 &  0.19 &   &  1.93 &  0.19 &  0.10 &  0.10 & +0.07 & +0.10 & -0.01 & +0.01 \\
DELVE~1-S1 & 4501.27 &  22.1 &  1.12 & -0.77 &  92.5 &  2.2 &  0.17 &   &  2.04 &  0.20 &  0.05 &  0.10 & +0.07 & +0.10 & -0.11 & +0.00 \\
DELVE~1-S1 & 4571.97 &  22.1 &  1.57 & -0.31 &  94.2 &  2.4 &  0.19 &   &  2.13 &  0.20 &  0.06 &  0.10 & +0.06 & +0.10 & -0.11 & +0.01 \\
DELVE~1-S1 & 4657.20 &  22.1 &  1.24 & -2.29 &   9.6 &  2.4 &  0.11 &   &  1.99 &  0.19 &  0.11 &  0.10 & +0.07 & +0.10 & -0.00 & +0.01 \\
DELVE~1-S1 & 5185.90 &  22.1 &  1.89 & -1.41 &  21.3 &  4.9 &  0.21 &   &  2.21 &  0.19 &  0.12 &  0.10 & +0.05 & +0.10 & -0.01 & +0.01 \\
DELVE~1-S1 & 5188.69 &  22.1 &  1.58 & -1.05 &  55.9 &  5.1 &  0.22 &   &  2.12 &  0.18 &  0.08 &  0.10 & +0.06 & +0.10 & -0.03 & +0.01 \\
DELVE~1-S1 & 5226.54 &  22.1 &  1.57 & -1.26 &  34.5 &  3.9 &  0.20 &   &  1.97 &  0.17 &  0.07 &  0.10 & +0.06 & +0.10 & -0.01 & +0.01 \\
DELVE~1-S1 & 5381.02 &  22.1 &  1.57 & -1.97 &  20.7 &  4.8 &  0.27 &   &  2.38 &  0.20 &  0.12 &  0.10 & +0.06 & +0.10 & -0.01 & +0.01 \\
DELVE~1-S1 & 4646.15 &  24.0 &  1.03 & -0.74 &  23.3 &  2.8 &  0.15 &   &  2.67 &  0.18 &  0.06 &  0.10 & +0.14 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 4651.28 &  24.0 &  0.98 & -1.46 &   9.8 &  3.0 &  0.17 &   &  2.89 &  0.22 &  0.13 &  0.10 & +0.14 & -0.02 & -0.00 & +0.00 \\
DELVE~1-S1 & 5298.28 &  24.0 &  0.98 & -1.14 &  16.6 &  3.6 &  0.15 &   &  2.79 &  0.20 &  0.10 &  0.10 & +0.14 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 5409.77 &  24.0 &  1.03 & -0.67 &  28.4 &  3.3 &  0.15 &   &  2.66 &  0.19 &  0.07 &  0.10 & +0.15 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 4558.64 &  24.1 &  4.07 & -0.43 &  18.8 &  2.7 &  0.16 &   &  2.76 &  0.17 &  0.07 &  0.10 & -0.01 & +0.11 & -0.01 & +0.01 \\
DELVE~1-S1 & 3949.95 &  26.0 &  2.18 & -1.25 &  47.8 &  4.9 &  0.10 &   &  4.53 &  0.20 &  0.09 &  0.10 & +0.14 & -0.02 & -0.03 & +0.00 \\
DELVE~1-S1 & 3977.74 &  26.0 &  2.20 & -1.12 &  70.3 &  5.5 &  0.19 &   &  4.83 &  0.22 &  0.12 &  0.10 & +0.13 & -0.02 & -0.08 & -0.00 \\
DELVE~1-S1 & 4067.98 &  26.0 &  3.21 & -0.53 &  30.8 &  3.5 &  0.13 &   &  4.64 &  0.17 &  0.07 &  0.10 & +0.11 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 4233.60 &  26.0 &  2.48 & -0.60 &  70.7 &  3.4 &  0.16 &   &  4.59 &  0.19 &  0.07 &  0.10 & +0.13 & -0.03 & -0.07 & +0.00 \\
DELVE~1-S1 & 4430.61 &  26.0 &  2.22 & -1.73 &  30.8 &  2.9 &  0.14 &   &  4.70 &  0.18 &  0.06 &  0.10 & +0.14 & -0.02 & -0.02 & +0.00 \\
DELVE~1-S1 & 4443.19 &  26.0 &  2.86 & -1.04 &  30.0 &  3.1 &  0.16 &   &  4.71 &  0.17 &  0.06 &  0.10 & +0.12 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 4466.55 &  26.0 &  2.83 & -0.60 &  60.3 &  2.3 &  0.18 &   &  4.77 &  0.17 &  0.04 &  0.10 & +0.12 & -0.03 & -0.05 & +0.00 \\
DELVE~1-S1 & 4494.56 &  26.0 &  2.20 & -1.14 &  58.5 &  2.6 &  0.17 &   &  4.56 &  0.18 &  0.05 &  0.10 & +0.14 & -0.02 & -0.04 & +0.00 \\
DELVE~1-S1 & 4531.15 &  26.0 &  1.48 & -2.10 &  60.8 &  2.6 &  0.17 &   &  4.73 &  0.20 &  0.05 &  0.10 & +0.16 & -0.03 & -0.05 & +0.00 \\
DELVE~1-S1 & 4592.65 &  26.0 &  1.56 & -2.46 &  31.4 &  2.3 &  0.15 &   &  4.67 &  0.19 &  0.04 &  0.10 & +0.16 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 4602.94 &  26.0 &  1.49 & -2.21 &  51.2 &  3.7 &  0.16 &   &  4.69 &  0.20 &  0.06 &  0.10 & +0.16 & -0.02 & -0.03 & +0.00 \\
DELVE~1-S1 & 4647.43 &  26.0 &  2.95 & -1.35 &  14.9 &  2.0 &  0.19 &   &  4.72 &  0.17 &  0.06 &  0.10 & +0.12 & -0.02 & -0.00 & +0.00 \\
DELVE~1-S1 & 4668.13 &  26.0 &  3.27 & -1.08 &  11.7 &  2.0 &  0.15 &   &  4.69 &  0.17 &  0.08 &  0.10 & +0.11 & -0.02 & -0.00 & +0.00 \\
DELVE~1-S1 & 4733.59 &  26.0 &  1.49 & -2.99 &  24.4 &  2.7 &  0.19 &   &  4.97 &  0.20 &  0.06 &  0.10 & +0.16 & -0.03 & -0.01 & +0.00 \\
DELVE~1-S1 & 4736.77 &  26.0 &  3.21 & -0.67 &  33.4 &  2.6 &  0.20 &   &  4.78 &  0.16 &  0.05 &  0.10 & +0.11 & -0.02 & -0.02 & +0.00 \\
DELVE~1-S1 & 4871.32 &  26.0 &  2.87 & -0.34 &  68.4 &  3.0 &  0.19 &   &  4.66 &  0.18 &  0.05 &  0.10 & +0.13 & -0.02 & -0.06 & -0.00 \\
DELVE~1-S1 & 4872.14 &  26.0 &  2.88 & -0.57 &  50.7 &  3.1 &  0.17 &   &  4.60 &  0.17 &  0.05 &  0.10 & +0.12 & -0.02 & -0.03 & +0.00 \\
DELVE~1-S1 & 4890.76 &  26.0 &  2.88 & -0.38 &  55.5 &  2.1 &  0.18 &   &  4.49 &  0.17 &  0.04 &  0.10 & +0.12 & -0.02 & -0.04 & +0.00 \\
DELVE~1-S1 & 4891.49 &  26.0 &  2.85 & -0.11 &  76.0 &  3.1 &  0.20 &   &  4.54 &  0.19 &  0.06 &  0.10 & +0.13 & -0.02 & -0.07 & -0.00 \\
DELVE~1-S1 & 4903.31 &  26.0 &  2.88 & -0.89 &  29.3 &  3.4 &  0.21 &   &  4.54 &  0.17 &  0.07 &  0.10 & +0.12 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 4918.99 &  26.0 &  2.86 & -0.34 &  64.3 &  2.6 &  0.18 &   &  4.57 &  0.18 &  0.05 &  0.10 & +0.13 & -0.02 & -0.05 & +0.00 \\
DELVE~1-S1 & 4920.50 &  26.0 &  2.83 &  0.07 &  87.8 &  2.8 &  0.19 &   &  4.57 &  0.20 &  0.06 &  0.10 & +0.13 & -0.03 & -0.10 & -0.00 \\
DELVE~1-S1 & 4939.69 &  26.0 &  0.86 & -3.25 &  50.0 &  3.4 &  0.23 &   &  4.95 &  0.22 &  0.06 &  0.10 & +0.18 & -0.03 & -0.03 & +0.00 \\
DELVE~1-S1 & 4994.13 &  26.0 &  0.92 & -2.97 &  44.3 &  4.7 &  0.18 &   &  4.64 &  0.22 &  0.08 &  0.10 & +0.18 & -0.03 & -0.02 & +0.00 \\
DELVE~1-S1 & 5006.12 &  26.0 &  2.83 & -0.62 &  53.4 & 11.7 &  0.19 &   &  4.63 &  0.25 &  0.19 &  0.10 & +0.13 & -0.02 & -0.04 & +0.00 \\
DELVE~1-S1 & 5049.82 &  26.0 &  2.28 & -1.36 &  40.4 &  6.8 &  0.22 &   &  4.52 &  0.21 &  0.12 &  0.10 & +0.14 & -0.02 & -0.02 & +0.00 \\
DELVE~1-S1 & 5051.63 &  26.0 &  0.92 & -2.76 &  59.5 &  5.8 &  0.18 &   &  4.67 &  0.23 &  0.09 &  0.10 & +0.18 & -0.03 & -0.04 & +0.00 \\
DELVE~1-S1 & 5079.74 &  26.0 &  0.99 & -3.24 &  30.5 &  6.7 &  0.20 &   &  4.74 &  0.23 &  0.12 &  0.10 & +0.17 & -0.03 & -0.01 & +0.00 \\
DELVE~1-S1 & 5083.34 &  26.0 &  0.96 & -2.84 &  53.8 &  7.3 &  0.25 &   &  4.71 &  0.24 &  0.12 &  0.10 & +0.18 & -0.03 & -0.03 & +0.00 \\
DELVE~1-S1 & 5123.72 &  26.0 &  1.01 & -3.06 &  38.8 &  3.9 &  0.17 &   &  4.73 &  0.22 &  0.07 &  0.10 & +0.18 & -0.03 & -0.02 & +0.00 \\
DELVE~1-S1 & 5133.69 &  26.0 &  4.18 &  0.36 &  34.9 &  4.6 &  0.26 &   &  4.84 &  0.16 &  0.09 &  0.10 & +0.09 & -0.01 & -0.02 & +0.00 \\
DELVE~1-S1 & 5150.84 &  26.0 &  0.99 & -3.04 &  42.1 &  5.5 &  0.24 &   &  4.74 &  0.23 &  0.09 &  0.10 & +0.18 & -0.03 & -0.02 & +0.00 \\
DELVE~1-S1 & 5151.91 &  26.0 &  1.01 & -3.32 &  41.7 &  3.9 &  0.18 &   &  5.04 &  0.22 &  0.06 &  0.10 & +0.18 & -0.03 & -0.02 & +0.00 \\
DELVE~1-S1 & 5171.60 &  26.0 &  1.49 & -1.72 &  81.7 &  5.5 &  0.22 &   &  4.67 &  0.24 &  0.11 &  0.10 & +0.17 & -0.02 & -0.09 & -0.00 \\
DELVE~1-S1 & 5192.34 &  26.0 &  3.00 & -0.42 &  47.1 &  4.5 &  0.18 &   &  4.51 &  0.17 &  0.07 &  0.10 & +0.12 & -0.02 & -0.03 & +0.00 \\
DELVE~1-S1 & 5194.94 &  26.0 &  1.56 & -2.02 &  59.6 &  5.9 &  0.27 &   &  4.66 &  0.22 &  0.10 &  0.10 & +0.16 & -0.02 & -0.04 & +0.00 \\
DELVE~1-S1 & 5198.71 &  26.0 &  2.22 & -2.09 &  16.6 &  4.4 &  0.16 &   &  4.66 &  0.21 &  0.12 &  0.10 & +0.14 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 5216.27 &  26.0 &  1.61 & -2.08 &  60.9 &  4.9 &  0.25 &   &  4.80 &  0.21 &  0.08 &  0.10 & +0.16 & -0.02 & -0.04 & +0.00 \\
DELVE~1-S1 & 5217.39 &  26.0 &  3.21 & -1.07 &  21.5 &  2.9 &  0.19 &   &  4.89 &  0.17 &  0.07 &  0.10 & +0.11 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 5263.31 &  26.0 &  3.27 & -0.87 &  21.2 &  4.3 &  0.19 &   &  4.75 &  0.18 &  0.10 &  0.10 & +0.11 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 5266.56 &  26.0 &  3.00 & -0.38 &  56.5 &  4.7 &  0.23 &   &  4.62 &  0.18 &  0.08 &  0.10 & +0.12 & -0.02 & -0.04 & +0.00 \\
DELVE~1-S1 & 5281.79 &  26.0 &  3.04 & -0.83 &  22.7 &  4.0 &  0.15 &   &  4.49 &  0.18 &  0.09 &  0.10 & +0.12 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 5283.62 &  26.0 &  3.24 & -0.45 &  39.3 &  3.2 &  0.15 &   &  4.67 &  0.16 &  0.06 &  0.10 & +0.11 & -0.02 & -0.02 & +0.00 \\
DELVE~1-S1 & 5324.18 &  26.0 &  3.21 & -0.11 &  55.4 &  4.0 &  0.21 &   &  4.57 &  0.18 &  0.07 &  0.10 & +0.12 & -0.02 & -0.04 & +0.00 \\
DELVE~1-S1 & 5332.90 &  26.0 &  1.56 & -2.78 &  18.7 &  4.5 &  0.19 &   &  4.65 &  0.22 &  0.12 &  0.10 & +0.16 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 5339.93 &  26.0 &  3.27 & -0.63 &  29.5 &  4.4 &  0.22 &   &  4.70 &  0.18 &  0.09 &  0.10 & +0.11 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 5341.02 &  26.0 &  1.61 & -1.95 &  71.9 &  5.4 &  0.24 &   &  4.85 &  0.23 &  0.10 &  0.10 & +0.17 & -0.02 & -0.07 & -0.00 \\
DELVE~1-S1 & 5367.47 &  26.0 &  4.42 &  0.44 &  18.8 &  3.2 &  0.19 &   &  4.66 &  0.15 &  0.08 &  0.10 & +0.08 & -0.01 & -0.01 & +0.00 \\
DELVE~1-S1 & 5369.96 &  26.0 &  4.37 &  0.54 &  24.2 &  4.2 &  0.20 &   &  4.64 &  0.16 &  0.09 &  0.10 & +0.08 & -0.01 & -0.01 & +0.00 \\
DELVE~1-S1 & 5371.49 &  26.0 &  0.96 & -1.64 & 119.8 &  3.8 &  0.24 &   &  4.77 &  0.30 &  0.09 &  0.10 & +0.20 & -0.03 & -0.18 & -0.02 \\
DELVE~1-S1 & 5397.13 &  26.0 &  0.92 & -1.98 & 114.4 &  3.7 &  0.23 &   &  4.93 &  0.30 &  0.09 &  0.10 & +0.20 & -0.02 & -0.17 & -0.02 \\
DELVE~1-S1 & 5415.20 &  26.0 &  4.39 &  0.64 &  29.8 &  4.5 &  0.24 &   &  4.68 &  0.16 &  0.09 &  0.10 & +0.08 & -0.01 & -0.01 & +0.00 \\
DELVE~1-S1 & 5429.70 &  26.0 &  0.96 & -1.88 & 106.0 &  3.8 &  0.22 &   &  4.69 &  0.28 &  0.08 &  0.10 & +0.20 & -0.03 & -0.15 & -0.01 \\
DELVE~1-S1 & 5497.52 &  26.0 &  1.01 & -2.82 &  50.9 &  5.0 &  0.26 &   &  4.66 &  0.22 &  0.08 &  0.10 & +0.18 & -0.02 & -0.03 & +0.00 \\
DELVE~1-S1 & 5501.47 &  26.0 &  0.96 & -3.05 &  58.3 &  4.2 &  0.24 &   &  4.95 &  0.22 &  0.07 &  0.10 & +0.18 & -0.02 & -0.04 & -0.00 \\
DELVE~1-S1 & 5506.78 &  26.0 &  0.99 & -2.79 &  59.2 &  2.9 &  0.20 &   &  4.74 &  0.22 &  0.05 &  0.10 & +0.18 & -0.02 & -0.04 & +0.00 \\
DELVE~1-S1 & 5586.76 &  26.0 &  3.37 & -0.11 &  49.8 &  4.3 &  0.26 &   &  4.64 &  0.17 &  0.07 &  0.10 & +0.11 & -0.02 & -0.03 & -0.00 \\
DELVE~1-S1 & 5624.54 &  26.0 &  3.42 & -0.76 &  16.4 &  2.7 &  0.16 &   &  4.66 &  0.17 &  0.08 &  0.10 & +0.11 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 6065.48 &  26.0 &  2.61 & -1.41 &  25.2 &  4.1 &  0.30 &   &  4.60 &  0.19 &  0.09 &  0.10 & +0.13 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 6136.61 &  26.0 &  2.45 & -1.41 &  38.4 &  3.2 &  0.23 &   &  4.67 &  0.18 &  0.05 &  0.10 & +0.14 & -0.02 & -0.02 & +0.00 \\
DELVE~1-S1 & 6137.69 &  26.0 &  2.59 & -1.35 &  30.9 &  2.6 &  0.21 &   &  4.63 &  0.17 &  0.05 &  0.10 & +0.13 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 6191.56 &  26.0 &  2.43 & -1.42 &  38.9 &  2.9 &  0.25 &   &  4.66 &  0.18 &  0.05 &  0.10 & +0.14 & -0.02 & -0.02 & +0.00 \\
DELVE~1-S1 & 6230.72 &  26.0 &  2.56 & -1.28 &  27.1 &  2.7 &  0.18 &   &  4.45 &  0.18 &  0.06 &  0.10 & +0.14 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 6252.56 &  26.0 &  2.40 & -1.77 &  34.1 &  3.1 &  0.24 &   &  4.89 &  0.18 &  0.06 &  0.10 & +0.14 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 6393.60 &  26.0 &  2.43 & -1.58 &  31.3 &  2.8 &  0.24 &   &  4.67 &  0.18 &  0.05 &  0.10 & +0.14 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 6430.85 &  26.0 &  2.18 & -1.95 &  29.9 &  3.1 &  0.28 &   &  4.73 &  0.19 &  0.06 &  0.10 & +0.15 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 6494.98 &  26.0 &  2.40 & -1.24 &  52.3 &  2.8 &  0.24 &   &  4.65 &  0.18 &  0.05 &  0.10 & +0.14 & -0.02 & -0.03 & +0.00 \\
DELVE~1-S1 & 6592.91 &  26.0 &  2.73 & -1.47 &  22.2 &  2.9 &  0.25 &   &  4.70 &  0.18 &  0.07 &  0.10 & +0.13 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 6677.99 &  26.0 &  2.69 & -1.42 &  26.5 &  3.2 &  0.25 &   &  4.70 &  0.18 &  0.07 &  0.10 & +0.13 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 7511.02 &  26.0 &  4.18 &  0.12 &  30.0 &  2.6 &  0.32 &   &  4.89 &  0.14 &  0.05 &  0.10 & +0.09 & -0.01 & -0.01 & +0.00 \\
DELVE~1-S1 & 4491.41 &  26.1 &  2.86 & -2.71 &  23.2 &  2.9 &  0.17 &   &  4.62 &  0.16 &  0.07 &  0.10 & +0.02 & +0.10 & -0.01 & +0.01 \\
DELVE~1-S1 & 4508.28 &  26.1 &  2.86 & -2.42 &  39.5 &  1.9 &  0.16 &   &  4.66 &  0.15 &  0.03 &  0.10 & +0.02 & +0.10 & -0.02 & +0.01 \\
DELVE~1-S1 & 4515.34 &  26.1 &  2.84 & -2.60 &  40.6 &  2.7 &  0.20 &   &  4.83 &  0.15 &  0.05 &  0.10 & +0.02 & +0.10 & -0.02 & +0.01 \\
DELVE~1-S1 & 4555.89 &  26.1 &  2.83 & -2.40 &  43.9 &  2.1 &  0.16 &   &  4.68 &  0.15 &  0.04 &  0.10 & +0.02 & +0.10 & -0.02 & +0.01 \\
DELVE~1-S1 & 4576.34 &  26.1 &  2.84 & -2.95 &  17.7 &  3.0 &  0.19 &   &  4.68 &  0.16 &  0.08 &  0.10 & +0.02 & +0.10 & -0.01 & +0.01 \\
DELVE~1-S1 & 4620.52 &  26.1 &  2.83 & -3.21 &  12.0 &  1.9 &  0.12 &   &  4.74 &  0.17 &  0.07 &  0.10 & +0.02 & +0.11 & -0.00 & +0.01 \\
DELVE~1-S1 & 5234.63 &  26.1 &  3.22 & -2.18 &  40.3 &  4.5 &  0.19 &   &  4.79 &  0.17 &  0.08 &  0.10 & +0.01 & +0.11 & -0.02 & +0.01 \\
DELVE~1-S1 & 5276.00 &  26.1 &  3.20 & -2.01 &  43.9 &  3.8 &  0.18 &   &  4.66 &  0.16 &  0.06 &  0.10 & +0.01 & +0.11 & -0.02 & +0.01 \\
DELVE~1-S1 & 5476.90 &  28.0 &  1.83 & -0.78 &  29.4 &  3.4 &  0.18 &   &  2.90 &  0.19 &  0.07 &  0.10 & +0.15 & -0.02 & -0.01 & +0.00 \\
DELVE~1-S1 & 3961.52 &  13.0 &  0.01 & -0.03 &  syn  &  syn &  0.14 &   &  3.73 &  0.40 &  0.10 &  0.10 & +0.26 & -0.19 & -0.19 & -0.03 \\
DELVE~1-S1 & 3905.52 &  14.0 &  1.91 & -1.08 &  syn  &  syn &  0.14 &   &  5.42 &  0.93 &  0.21 &  0.10 & +0.27 & -0.58 & -0.49 & -0.41 \\
DELVE~1-S1 & 4102.94 &  14.0 &  1.91 & -3.03 &  syn  &  syn &  0.16 &   &  5.15 &  0.24 &  0.02 &  0.10 & +0.21 & -0.06 & -0.03 & +0.01 \\
DELVE~1-S1 & 4320.70 &  21.1 &  0.60 & -0.28 &  syn  &  syn &  0.16 &   &  0.18 &  0.38 &  0.08 &  0.10 & -0.20 & +0.29 & -0.06 & -0.02 \\
DELVE~1-S1 & 4374.50 &  21.1 &  0.62 & -0.46 &  syn  &  syn &  0.14 &   &  0.20 &  0.24 &  0.08 &  0.10 & -0.13 & +0.16 & -0.03 & -0.01 \\
DELVE~1-S1 & 4415.60 &  21.1 &  0.59 & -0.68 &  syn  &  syn &  0.16 &   &  0.29 &  0.18 &  0.07 &  0.10 & -0.00 & +0.13 & -0.02 & +0.00 \\
DELVE~1-S1 & 5657.90 &  21.1 &  1.51 & -0.54 &  syn  &  syn &  0.16 &   &  0.48 &  0.17 &  0.08 &  0.10 & +0.04 & +0.11 & -0.01 & +0.01 \\
DELVE~1-S1 & 3995.70 &  27.0 &  1.05 & -0.10 &  syn  &  syn &  0.14 &   &  2.26 &  0.20 &  0.13 &  0.10 & +0.05 & +0.09 & -0.03 & -0.02 \\
DELVE~1-S1 & 4118.80 &  27.0 &  1.05 & -0.48 &  syn  &  syn &  0.16 &   &  2.08 &  0.24 &  0.17 &  0.10 & +0.13 & -0.01 & -0.01 & -0.00 \\
DELVE~1-S1 & 4121.30 &  27.0 &  0.92 & -0.33 &  syn  &  syn &  0.14 &   &  2.03 &  0.19 &  0.12 &  0.10 & +0.11 & +0.00 & -0.00 & -0.00 \\
DELVE~1-S1 & 4077.71 &  38.1 &  0.00 &  0.15 &  syn  &  syn &  0.15 &   & -1.64 &  0.28 &  0.10 &  0.10 & -0.09 & +0.20 & -0.10 & -0.01 \\
DELVE~1-S1 & 4215.52 &  38.1 &  0.00 & -0.17 &  syn  &  syn &  0.14 &   & -1.44 &  0.38 &  0.11 &  0.10 & +0.31 & -0.15 & -0.04 & +0.04 \\
DELVE~1-S1 & 4554.00 &  56.1 &  0.00 &  0.17 &  syn  &  syn &  0.16 &   & -2.29 &  0.17 &  0.05 &  0.10 & +0.11 & +0.06 & +0.02 & +0.01 \\
DELVE~1-S1 & 4934.10 &  56.1 &  0.00 & -0.16 &  syn  &  syn &  0.15 &   & -2.20 &  0.18 &  0.07 &  0.10 & +0.09 & +0.10 & -0.00 & +0.01 \\
DELVE~1-S1 & 6141.70 &  56.1 &  0.70 & -0.08 &  syn  &  syn &  0.23 &   & -1.84 &  0.18 &  0.08 &  0.10 & +0.08 & +0.10 & +0.00 & +0.02 \\
DELVE~1-S1 & 6496.90 &  56.1 &  0.60 & -0.38 &  syn  &  syn &  0.24 &   & -1.67 &  0.17 &  0.07 &  0.10 & +0.08 & +0.09 & +0.01 & +0.02 \\
DELVE~1-S1 & 4313.00 & 106.0 &\nodata&\nodata&  syn  &  syn &  0.14 &   &  7.29 &  0.34 &  0.01 &  0.10 & +0.31 & -0.10 & +0.00 & +0.03 \\
DELVE~1-S1 & 4323.00 & 106.0 &\nodata&\nodata&  syn  &  syn &  0.16 &   &  7.22 &  0.32 &  0.02 &  0.10 & +0.28 & -0.11 & +0.01 & +0.02 \\
DELVE~1-S1 & 3876.00 & 607.0 &\nodata&\nodata&  syn  &  syn &  0.14 &   &  7.03 &  0.39 &  0.02 &  0.10 & +0.36 & -0.09 & +0.00 & +0.02 \\
DELVE~1-S1 & 4205.00 & 607.0 &\nodata&\nodata&  syn  &  syn &  0.16 &   &  7.13 &  0.38 &  0.05 &  0.10 & +0.35 & -0.08 & +0.01 & +0.02 \\
DELVE~1-S1 & 4129.70 &  63.1 &  0.00 &  0.22 &  syn  &  syn &\nodata&$<$& -1.78 &\nodata&\nodata&\nodata&\nodata&\nodata&\nodata&\nodata \\
Eri~III-S1 & 6300.30 &   8.0 &  0.00 & -9.69 &  29.2 &  5.1 &  0.23 &   &  7.76 &  0.22 &  0.09 &  0.10 & +0.16 & +0.08 & -0.01 & +0.02 \\
Eri~III-S1 & 7775.39 &   8.0 &  9.15 &  0.00 &  16.1 &  3.2 &  0.29 &   &  8.04 &  0.31 &  0.11 &  0.10 & -0.24 & +0.13 & -0.01 & -0.01 \\
Eri~III-S1 & 5889.95 &  11.0 &  0.00 &  0.11 & 189.7 &  6.3 &  0.33 &   &  4.00 &  0.38 &  0.07 &  0.10 & +0.32 & -0.11 & -0.12 & -0.01 \\
Eri~III-S1 & 5895.92 &  11.0 &  0.00 & -0.19 & 163.0 &  5.9 &  0.30 &   &  3.97 &  0.36 &  0.08 &  0.10 & +0.30 & -0.07 & -0.14 & -0.01 \\
Eri~III-S1 & 4702.99 &  12.0 &  4.33 & -0.44 & 102.7 &  6.9 &  0.21 &   &  5.61 &  0.23 &  0.09 &  0.10 & +0.16 & -0.07 & -0.06 & +0.00 \\
Eri~III-S1 & 5172.68 &  12.0 &  2.71 & -0.36 & 195.0 & 16.4 &  0.31 &   &  5.02 &  0.39 &  0.14 &  0.10 & +0.31 & -0.14 & -0.09 & +0.00 \\
Eri~III-S1 & 5183.60 &  12.0 &  2.72 & -0.17 & 243.0 & 13.2 &  0.36 &   &  5.18 &  0.39 &  0.07 &  0.10 & +0.33 & -0.17 & -0.05 & +0.01 \\
Eri~III-S1 & 5528.40 &  12.0 &  4.35 & -0.55 &  77.5 &  6.5 &  0.24 &   &  5.41 &  0.20 &  0.09 &  0.10 & +0.14 & -0.03 & -0.04 & +0.00 \\
Eri~III-S1 & 5711.09 &  12.0 &  4.35 & -1.84 &  22.4 &  5.2 &  0.22 &   &  5.83 &  0.20 &  0.12 &  0.10 & +0.12 & -0.01 & -0.01 & +0.00 \\
Eri~III-S1 & 7664.90 &  19.0 &  0.00 &  0.13 &  58.9 & 14.8 &  0.51 &   &  2.92 &  0.31 &  0.22 &  0.10 & +0.19 & -0.01 & -0.04 & +0.00 \\
Eri~III-S1 & 7698.96 &  19.0 &  0.00 & -0.18 &  41.3 &  7.3 &  0.54 &   &  2.96 &  0.25 &  0.12 &  0.10 & +0.19 & -0.01 & -0.02 & +0.00 \\
Eri~III-S1 & 4435.69 &  20.0 &  1.89 & -0.53 &  32.8 & 10.2 &  0.17 &   &  3.79 &  0.27 &  0.18 &  0.10 & +0.17 & -0.02 & -0.02 & +0.00 \\
Eri~III-S1 & 6122.22 &  20.0 &  1.89 & -0.34 &  16.6 &  3.9 &  0.22 &   &  3.14 &  0.23 &  0.11 &  0.10 & +0.18 & -0.02 & -0.01 & +0.00 \\
Eri~III-S1 & 6162.17 &  20.0 &  1.90 & -0.12 &  40.2 &  4.8 &  0.28 &   &  3.43 &  0.22 &  0.08 &  0.10 & +0.18 & -0.02 & -0.02 & +0.00 \\
Eri~III-S1 & 6439.07 &  20.0 &  2.52 &  0.39 &  26.4 &  4.8 &  0.27 &   &  3.37 &  0.21 &  0.10 &  0.10 & +0.15 & -0.01 & -0.01 & +0.00 \\
Eri~III-S1 & 4443.80 &  22.1 &  1.08 & -0.71 &  90.2 &  9.3 &  0.20 &   &  2.05 &  0.29 &  0.20 &  0.10 & +0.12 & +0.08 & -0.12 & +0.01 \\
Eri~III-S1 & 4501.27 &  22.1 &  1.12 & -0.77 &  62.8 &  7.0 &  0.16 &   &  1.65 &  0.21 &  0.12 &  0.10 & +0.11 & +0.08 & -0.05 & +0.01 \\
Eri~III-S1 & 4571.97 &  22.1 &  1.57 & -0.31 & 102.4 &  8.4 &  0.22 &   &  2.46 &  0.30 &  0.19 &  0.10 & +0.10 & +0.08 & -0.16 & +0.00 \\
Eri~III-S1 & 5188.69 &  22.1 &  1.58 & -1.05 &  46.3 &  9.4 &  0.21 &   &  2.15 &  0.22 &  0.15 &  0.10 & +0.09 & +0.08 & -0.03 & +0.01 \\
Eri~III-S1 & 5409.77 &  24.0 &  1.03 & -0.67 &  46.1 & 10.8 &  0.25 &   &  2.84 &  0.33 &  0.17 &  0.10 & +0.26 & -0.02 & -0.03 & +0.00 \\
Eri~III-S1 & 4233.60 &  26.0 &  2.48 & -0.60 &  54.8 & 11.1 &  0.13 &   &  4.18 &  0.32 &  0.19 &  0.10 & +0.23 & -0.02 & -0.04 & +0.00 \\
Eri~III-S1 & 4466.55 &  26.0 &  2.83 & -0.60 &  46.6 & 11.7 &  0.21 &   &  4.43 &  0.31 &  0.20 &  0.10 & +0.21 & -0.02 & -0.03 & +0.00 \\
Eri~III-S1 & 4494.56 &  26.0 &  2.20 & -1.14 &  50.5 &  8.8 &  0.19 &   &  4.30 &  0.30 &  0.14 &  0.10 & +0.24 & -0.02 & -0.04 & +0.00 \\
Eri~III-S1 & 4531.15 &  26.0 &  1.48 & -2.10 &  61.8 & 12.0 &  0.24 &   &  4.60 &  0.37 &  0.21 &  0.10 & +0.28 & -0.02 & -0.05 & +0.00 \\
Eri~III-S1 & 4602.94 &  26.0 &  1.49 & -2.21 &  50.6 &  8.4 &  0.19 &   &  4.54 &  0.33 &  0.13 &  0.10 & +0.28 & -0.02 & -0.04 & +0.00 \\
Eri~III-S1 & 4871.32 &  26.0 &  2.87 & -0.34 &  38.8 &  7.0 &  0.19 &   &  4.04 &  0.26 &  0.12 &  0.10 & +0.21 & -0.02 & -0.02 & +0.00 \\
Eri~III-S1 & 4872.14 &  26.0 &  2.88 & -0.57 &  41.8 &  6.2 &  0.16 &   &  4.34 &  0.25 &  0.10 &  0.10 & +0.21 & -0.02 & -0.02 & +0.00 \\
Eri~III-S1 & 4890.76 &  26.0 &  2.88 & -0.38 &  57.9 &  6.3 &  0.17 &   &  4.41 &  0.26 &  0.10 &  0.10 & +0.21 & -0.02 & -0.04 & +0.00 \\
Eri~III-S1 & 4891.49 &  26.0 &  2.85 & -0.11 &  72.8 &  6.6 &  0.20 &   &  4.35 &  0.28 &  0.12 &  0.10 & +0.22 & -0.02 & -0.07 & +0.00 \\
Eri~III-S1 & 4918.99 &  26.0 &  2.86 & -0.34 &  52.9 & 13.1 &  0.28 &   &  4.26 &  0.32 &  0.21 &  0.10 & +0.22 & -0.02 & -0.04 & +0.00 \\
Eri~III-S1 & 4939.69 &  26.0 &  0.86 & -3.25 &  46.8 &  7.5 &  0.18 &   &  4.74 &  0.35 &  0.12 &  0.10 & +0.31 & -0.02 & -0.03 & +0.01 \\
Eri~III-S1 & 5006.12 &  26.0 &  2.83 & -0.62 &  32.7 & 10.7 &  0.20 &   &  4.16 &  0.31 &  0.19 &  0.10 & +0.22 & -0.02 & -0.02 & +0.01 \\
Eri~III-S1 & 5049.82 &  26.0 &  2.28 & -1.36 &  75.5 & 11.4 &  0.21 &   &  4.98 &  0.35 &  0.21 &  0.10 & +0.25 & -0.01 & -0.08 & +0.00 \\
Eri~III-S1 & 5171.60 &  26.0 &  1.49 & -1.72 &  62.4 & 12.0 &  0.23 &   &  4.18 &  0.36 &  0.20 &  0.10 & +0.28 & -0.02 & -0.06 & +0.00 \\
Eri~III-S1 & 5191.45 &  26.0 &  3.04 & -0.55 &  35.5 & 10.2 &  0.22 &   &  4.37 &  0.29 &  0.17 &  0.10 & +0.21 & -0.02 & -0.02 & +0.00 \\
Eri~III-S1 & 5192.34 &  26.0 &  3.00 & -0.42 &  50.8 &  9.2 &  0.22 &   &  4.45 &  0.28 &  0.15 &  0.10 & +0.21 & -0.02 & -0.03 & +0.00 \\
Eri~III-S1 & 5194.94 &  26.0 &  1.56 & -2.02 &  61.9 & 10.1 &  0.25 &   &  4.55 &  0.35 &  0.17 &  0.10 & +0.28 & -0.01 & -0.05 & +0.00 \\
Eri~III-S1 & 5232.94 &  26.0 &  2.94 & -0.06 &  77.2 & 11.3 &  0.27 &   &  4.45 &  0.33 &  0.20 &  0.10 & +0.23 & -0.02 & -0.08 & +0.00 \\
Eri~III-S1 & 5266.56 &  26.0 &  3.00 & -0.38 &  36.2 & 10.4 &  0.25 &   &  4.17 &  0.30 &  0.18 &  0.10 & +0.21 & -0.02 & -0.02 & +0.00 \\
Eri~III-S1 & 5283.62 &  26.0 &  3.24 & -0.45 &  32.7 &  9.8 &  0.29 &   &  4.45 &  0.28 &  0.17 &  0.10 & +0.20 & -0.02 & -0.02 & +0.00 \\
Eri~III-S1 & 5324.18 &  26.0 &  3.21 & -0.11 &  48.8 & 10.4 &  0.25 &   &  4.35 &  0.28 &  0.17 &  0.10 & +0.20 & -0.02 & -0.03 & +0.00 \\
Eri~III-S1 & 5339.93 &  26.0 &  3.27 & -0.63 &  22.9 &  6.6 &  0.14 &   &  4.45 &  0.26 &  0.14 &  0.10 & +0.19 & -0.02 & -0.01 & +0.00 \\
Eri~III-S1 & 5341.02 &  26.0 &  1.61 & -1.95 &  42.2 &  7.4 &  0.20 &   &  4.22 &  0.32 &  0.12 &  0.10 & +0.28 & -0.02 & -0.02 & +0.01 \\
Eri~III-S1 & 5405.77 &  26.0 &  0.99 & -1.85 &  88.8 &  9.2 &  0.26 &   &  4.16 &  0.41 &  0.19 &  0.10 & +0.33 & -0.01 & -0.11 & -0.00 \\
Eri~III-S1 & 5429.70 &  26.0 &  0.96 & -1.88 &  96.0 &  7.6 &  0.24 &   &  4.29 &  0.40 &  0.15 &  0.10 & +0.33 & -0.01 & -0.14 & -0.00 \\
Eri~III-S1 & 5434.52 &  26.0 &  1.01 & -2.13 &  76.9 &  8.6 &  0.27 &   &  4.24 &  0.38 &  0.16 &  0.10 & +0.32 & -0.01 & -0.08 & +0.00 \\
Eri~III-S1 & 5501.47 &  26.0 &  0.96 & -3.05 &  38.9 & 11.7 &  0.34 &   &  4.49 &  0.38 &  0.19 &  0.10 & +0.31 & -0.02 & -0.02 & +0.01 \\
Eri~III-S1 & 5506.78 &  26.0 &  0.99 & -2.79 &  64.7 & 10.6 &  0.33 &   &  4.67 &  0.38 &  0.18 &  0.10 & +0.31 & -0.01 & -0.05 & +0.00 \\
Eri~III-S1 & 6065.48 &  26.0 &  2.61 & -1.41 &  16.1 &  4.3 &  0.20 &   &  4.25 &  0.28 &  0.12 &  0.10 & +0.23 & -0.02 & -0.01 & +0.00 \\
Eri~III-S1 & 6136.61 &  26.0 &  2.45 & -1.41 &  24.6 &  3.9 &  0.23 &   &  4.28 &  0.27 &  0.08 &  0.10 & +0.24 & -0.02 & -0.01 & +0.00 \\
Eri~III-S1 & 6137.69 &  26.0 &  2.59 & -1.35 &  24.5 &  5.4 &  0.26 &   &  4.38 &  0.27 &  0.11 &  0.10 & +0.23 & -0.02 & -0.01 & +0.00 \\
Eri~III-S1 & 6191.56 &  26.0 &  2.43 & -1.42 &  40.1 &  9.6 &  0.39 &   &  4.57 &  0.31 &  0.16 &  0.10 & +0.24 & -0.02 & -0.02 & +0.00 \\
Eri~III-S1 & 6230.72 &  26.0 &  2.56 & -1.28 &  24.8 &  4.9 &  0.30 &   &  4.28 &  0.27 &  0.11 &  0.10 & +0.23 & -0.01 & -0.01 & +0.00 \\
Eri~III-S1 & 6252.56 &  26.0 &  2.40 & -1.77 &  26.5 &  3.9 &  0.24 &   &  4.62 &  0.27 &  0.08 &  0.10 & +0.24 & -0.01 & -0.01 & +0.00 \\
Eri~III-S1 & 6393.60 &  26.0 &  2.43 & -1.58 &  42.8 &  5.6 &  0.37 &   &  4.76 &  0.28 &  0.09 &  0.10 & +0.24 & -0.01 & -0.02 & +0.00 \\
Eri~III-S1 & 6430.85 &  26.0 &  2.18 & -1.95 &  31.4 &  5.2 &  0.33 &   &  4.63 &  0.29 &  0.10 &  0.10 & +0.25 & -0.01 & -0.01 & +0.00 \\
Eri~III-S1 & 6494.98 &  26.0 &  2.40 & -1.24 &  46.6 &  4.3 &  0.31 &   &  4.44 &  0.28 &  0.07 &  0.10 & +0.25 & -0.01 & -0.03 & +0.00 \\
Eri~III-S1 & 6677.99 &  26.0 &  2.69 & -1.42 &  41.8 &  6.5 &  0.51 &   &  4.87 &  0.27 &  0.11 &  0.10 & +0.23 & -0.01 & -0.02 & +0.00 \\
Eri~III-S1 & 4555.89 &  26.1 &  2.83 & -2.40 &  20.5 &  7.4 &  0.15 &   &  4.41 &  0.22 &  0.17 &  0.10 & +0.03 & +0.09 & -0.01 & +0.01 \\
Eri~III-S1 & 4583.83 &  26.1 &  2.81 & -1.94 &  43.0 &  9.0 &  0.22 &   &  4.38 &  0.21 &  0.15 &  0.10 & +0.03 & +0.09 & -0.03 & +0.01 \\
Eri~III-S1 & 5476.90 &  28.0 &  1.83 & -0.78 &  36.3 &  7.1 &  0.21 &   &  2.91 &  0.30 &  0.12 &  0.10 & +0.25 & -0.01 & -0.02 & +0.00 \\
Eri~III-S1 & 3961.52 &  13.0 &  0.01 & -0.03 &  syn  &  syn &  0.17 &   &  3.56 &  0.99 &  0.49 &  0.10 & +0.40 & -0.60 & -0.44 & -0.12 \\
Eri~III-S1 & 4102.94 &  14.0 &  1.91 & -3.03 &  syn  &  syn &  0.12 &   &  4.87 &  0.59 &  0.54 &  0.10 & +0.22 & -0.01 & -0.03 & +0.01 \\
Eri~III-S1 & 4320.70 &  21.1 &  0.60 & -0.28 &  syn  &  syn &  0.22 &   &  0.29 &  0.38 &  0.32 &  0.10 & +0.12 & +0.11 & -0.07 & +0.01 \\
Eri~III-S1 & 4400.40 &  21.1 &  0.60 & -0.54 &  syn  &  syn &  0.18 &   &  0.62 &  0.50 &  0.28 &  0.10 & -0.24 & +0.31 & -0.05 & -0.04 \\
Eri~III-S1 & 4415.60 &  21.1 &  0.59 & -0.68 &  syn  &  syn &  0.19 &   &  0.14 &  0.39 &  0.36 &  0.10 & -0.07 & +0.10 & -0.02 & -0.01 \\
Eri~III-S1 & 4077.71 &  38.1 &  0.00 &  0.15 &  syn  &  syn &  0.14 &   & -2.11 &  0.60 &  0.54 &  0.10 & +0.23 & +0.04 & -0.04 & +0.04 \\
Eri~III-S1 & 4554.00 &  56.1 &  0.00 &  0.17 &  syn  &  syn &  0.18 &   & -1.93 &  0.25 &  0.18 &  0.10 & +0.12 & +0.09 & -0.00 & -0.00 \\
Eri~III-S1 & 4934.10 &  56.1 &  0.00 & -0.16 &  syn  &  syn &  0.17 &   & -1.70 &  0.32 &  0.24 &  0.10 & +0.17 & +0.09 & -0.01 & +0.01 \\
Eri~III-S1 & 6496.90 &  56.1 &  0.60 & -0.38 &  syn  &  syn &  0.24 &   & -1.45 &  0.26 &  0.15 &  0.10 & +0.18 & +0.05 & -0.00 & +0.02 \\
Eri~III-S1 & 4313.00 & 106.0 &\nodata&\nodata&  syn  &  syn &  0.22 &   &  7.17 &  0.37 &  0.06 &  0.10 & +0.35 & -0.00 & -0.00 & +0.02 \\
Eri~III-S1 & 4323.00 & 106.0 &\nodata&\nodata&  syn  &  syn &  0.21 &   &  7.09 &  0.35 &  0.07 &  0.10 & +0.32 & -0.05 & -0.01 & +0.02 \\
Eri~III-S1 & 4205.00 & 607.0 &\nodata&\nodata&  syn  &  syn &  0.19 &   &  7.31 &  0.48 &  0.04 &  0.10 & +0.46 & -0.04 & +0.00 & +0.03 \\
Eri~III-S1 & 4129.70 &  63.1 &  0.00 &  0.22 &  syn  &  syn &\nodata&$<$& -0.61 &\nodata&\nodata&\nodata&\nodata&\nodata&\nodata&\nodata \\
\enddata
\tablecomments{A portion of this table is shown for form. The full
  version is available online. The columns are wavelength ($\lambda$), species (ID), excitation potential ($\chi$), cross section ($\log gf$), equivalent width and uncertainty (EW and $\sigma$(EW)), full width half max (FWHM), upper limit flag (ul), line abundance and total uncertainty ($\log \epsilon_i$, $\sigma_i$), statistical uncertainty ($e_i$), per-line systematic uncertainty $s_X$, and errors due to stellar parameter uncertainties ($\delta_{i,\teff}$, $\delta_{i,\logg}$, $\delta_{i,\nu_t}$, $\delta_{i,\text{[M/H]}}$). The total uncertainty $\sigma_i$ is the quadrature sum of $e_i$, $s_X$, $\delta_{i,\teff}$, $\delta_{i,\logg}$, $\delta_{i,\nu_t}$, and $\delta_{i,\text{[M/H]}}$.}
\end{deluxetable*}

